First Tree-like Quantum Data Structure: Quantum B+ Tree

Quantum computing is a popular topic in computer science, which has recently attracted many studies in various areas such as machine learning and network. However, the topic of quantum data structures seems neglected. There is an open problem in the database area: Can we improve existing data structures by quantum techniques? Consider a dataset of key-record pairs. Given an interval as a query range, a classical B+ tree can report all the records with keys within this interval, which is called a range query, in O(log N + k) time, where N is the total number of records and k is the output size. It is asymptotically optimal in a classical computer but not efficient enough in a quantum computer, because it is expected that the execution time and the output size are linear in a quantum computer. In this paper, we propose the quantum range query problem. Different from the classical range queries, a quantum range query returns the results in quantum bits, which has broad potential applications due to the foreseeable advance of quantum computers and quantum algorithms. To the best of our knowledge, we design the first tree-like quantum data structure called the quantum B+ tree. Based on this data structure, we propose a hybrid quantum-classical algorithm to do the range search. It answers a static quantum range query in O(log_B N) time, which is asymptotically optimal in quantum computers. Since the execution time does not depend on the output size (i.e., k, which could be as large as O(N)), it is significantly faster than the classical data structure. Moreover, we extend our quantum B+ tree to answer the dynamic and d-dimensional quantum range queries efficiently in O(log^2_B N) and O(log^d_B N) time, respectively. Our experimental results show that our proposed quantum data structures achieve up to 1000x improvement in the number of memory accesses compared to their classical competitors.

==> _old_sections/prev-algorithm.tex <==
\section{Quantum B+ Tree}\label{alg}
In this section, we propose the quantum B+ tree to solve the quantum range query problem. In Section \ref{static}, for static quantum range query, we introduce how to store a static quantum B+ tree in a QRAM, and give the algorithms for bulk-loadings and range queries. Then, we discuss two variants of the static quantum B+ tree. The first one in Section \ref{dynamic} is the dynamic quantum B+ tree for dynamic quantum range query, which supports two more kinds of operations: Insertions and deletions. The second one in Section \ref{range} is the static quantum range tree for high-dimensional static quantum range query, which is based on the static quantum B+ tree.

\subsection{Static Quantum B+ Tree}\label{static}

\begin{figure*}[tbp]
  \centering
  \subfigure{
  \includegraphics[width=0.9\textwidth]{figure/static.pdf}}
  \caption{An example of a quantum B+ tree: $N=14$ and $B=4$}
  \label{fig:staticexp}
\end{figure*}


In our design, a static quantum B+ tree has two parts: A classical part and a quantum part. 

The classical part is stored in either a classical computer or a quantum computer, since it can be regarded as a quantum system only using $\ket{0}$ and $\ket{1}$ without any superposition. It is based on a weight-balanced B+ tree \cite{arge1996optimal}. A weight-balanced B+ tree is a tree data structure that consists of internal nodes and leaves. Each node has a unique ID number, which can be expressed by $n_i$ bits. A user parameter $B$ is a constant in the B+ tree, which is the branching factor usually set by the block size. We assume that $B$ is a power of $2$ and $B\geq 4$, which means there exists a constant integer $n_b\geq 2$ such that $B=2^{n_b}$. A leaf node contains $B$ key-record pairs sorted by the keys. An internal node has $B$ children $c_0, c_1,\cdots, c_{B-1}$ and $B$ routing keys $(l_0,r_0), (l_1,r_1), \cdots, (l_{B-1},r_{B-1})$ where $l_i$ is the least key in the subtree of $c_i$, and $r_i$ is the largest key in the subtree of $c_i$.  A node or a key-record pair can be empty, which is stored as a special mark $dummy$. In practice, $dummy$ can be the maximum number of the data type so that it will always be sorted to the last positions. We have the following definitions.
\begin{itemize}
	\item The level of a tree node is the distance from the root. All the leaves are in the same level.
	\item The height of a tree node is the distance from the leaves. The height of the tree is the height of the root node.
	\item The weight of a tree node is defined to be the number of non-dummy key-record pairs below the node. If a non-root node of height $h$ has a weight between $\frac{1}{4}B^{h+1}$ and $B^{h+1}$, then the node is \emph{balanced}. Moreover, if the non-root node of height $h$ has a weight between $\frac{1}{2}B^{h+1}$ and $B^{h+1}$, then the node is \emph{perfectly balanced}. If all the non-dummy node is perfectly balanced, then the B+ tree is perfectly balanced.
\end{itemize}
In a static quantum B+ tree, each non-root node has between $B/4$ and $B$ non-dummy children, and the root node has at least two non-dummy children, so the height of the tree is $O(\log_B N)$. 

The quantum part is stored in $2$ QRAMs $\mathcal{Q}_0$ and $\mathcal{Q}_1$. The first QRAM $\mathcal{Q}_0$ is to store the mapping from the internal nodes to their children.  Consider an internal node $u$ in the classical part has $B$ children $c_0,\cdots, c_{B-1}$ which contains $f$ non-dummy children $u_0,\cdots, u_{f-1}$ followed by $B-f$ $dummies$. In the quantum part, $c_0, c_1, \cdots, c_{B-1}$ are stored in $\mathcal{Q}_0[u*B+0], \mathcal{Q}_0[u*B+1],\cdots, \mathcal{Q}_0[u*B+B-1]$ such that 
\begin{align*}
 &\mathcal{Q}_0\frac{1}{\sqrt{B}}\sum_{i=0}^{B-1}\ket{u}\ket{i}\ket{0}
 =\frac{1}{\sqrt{B}}\sum_{i=0}^{B-1}\ket{u*B+i}\ket{c_i}\\
 =&\frac{1}{\sqrt{B}}\sum_{i=0}^{f-1}\ket{u*B+i}\ket{u_i}+\frac{1}{\sqrt{B}}\sum_{i=f}^{B-1}\ket{u*B+i}\ket{dummy}\\
 =&\frac{1}{\sqrt{B}}\sum_{i=0}^{f-1}\ket{u}\ket{i}\ket{u_i}+\frac{1}{\sqrt{B}}\sum_{i=f}^{B-1}\ket{u}\ket{i}\ket{dummy}.
\end{align*}
Then, if we only consider the first $n_i$ qubits and the last $n_i$ qubits, we obtain a quantum transformation 
$\ket{u}\ket{0}\rightarrow \frac{1}{\sqrt{B}}\sum_{i=0}^{f-1}\ket{u}\ket{u_i}+\frac{\sqrt{B-f}}{\sqrt{B}}\ket{u}\ket{dummy}.$
By the above quantum transformation, we can read out the IDs of all the children of the node $u$ by only one memory access. Consider a leaf node $u$ with no children. We define that for each $i\in[0,B-1]$, $\mathcal{Q}_0[u*B+i]=u$. The second QRAM $\mathcal{Q}_1$ is to store the mapping from the leaves to the key-record pairs. Consider a leaf node $u$ in the classical part has $B$ key-record pairs which contains $f$ non-dummy key-record pairs $(key_0, rec_0),\cdots, (key_{f-1},$ $rec_{f-1})$ followed by $B-f$ $dummies$. Similarly, in the quantum part, $(key_0, rec_0),\cdots, (key_{f-1}, rec_{f-1})$ and $B-f$ $dummies$ are stored in $\mathcal{Q}_1[u*B+0], \mathcal{Q}_1[u*B+1],\cdots, \mathcal{Q}_1[u*B+B-1]$ such that
\begin{align*}
 &\mathcal{Q}_1\frac{1}{\sqrt{B}}\sum_{i=0}^{B-1}\ket{u}\ket{i}\ket{0}\\
 =&\frac{1}{\sqrt{B}}\sum_{i=0}^{f-1}\ket{u}\ket{i}\ket{key_i}\ket{rec_i}+\frac{1}{\sqrt{B}}\sum_{i=f}^{B-1}\ket{u}\ket{i}\ket{dummy}.
\end{align*}
Specially, for a dummy node, we define that for each $i\in [0, B-1]$, we have $\mathcal{Q}_0[dummy*B+i]=dummy$ and $\mathcal{Q}_1[dummy*B+i]=dummy$. Figure \ref{fig:staticexp} shows an example of a quantum B+ tree stored in a quantum computer. The left side of the vertical line is the classical part. There is a classical weight-balanced B+ tree with $N=14$ and $B=4$. Each box is a node in the tree where the big number is the node ID. An internal node has $4$ children and it has a pair of bounds $(l_i, r_i)$ for each non-dummy child. A leaf node has $4$ key-record pairs. The right side of the vertical line is the quantum part. $\mathcal{Q}_0$ is to store the edges. For example, node $1$, node $2$, node $3$ and $dummy$ are $4$ children of node $0$, so we have $\mathcal{Q}_0[0*4+0]=1$, $\mathcal{Q}_0[0*4+1]=2$, $\mathcal{Q}_0[0*4+2]=3$ and $\mathcal{Q}_0[0*4+3]=dummy$. Since node $10$ is a leaf node, we have $\mathcal{Q}_0[10*4+i]=10$ for $i\in [0, 3]$, and $\mathcal{Q}_1[10*4+0]=(33,rec_{33})$.

To analyze the cost of building a quantum B+ tree, we have the following Theorem \ref{theo1}.

\begin{theorem}\label{theo1}
\vspace{-1mm}
Given a list of $N$ key-record pairs sorted by the keys, a perfectly balanced quantum B+ tree can be built in $O(N)$ time.
\vspace{-1mm}
\end{theorem}
\begin{proof}
Let $h=\lfloor \log_B N \rfloor$. First, we evenly distribute the $N$ key-record pairs into $\lceil N/B^h \rceil \cdot B^{h-1}$ leaves. Then, we build the tree from the bottom to the top, starting from the leaves. Since there are $O(N)$ leaves, there are $O(N)$ internal nodes, so the building costs $O(N)$ time. When building the B+ tree, we need to update the QRAM to make the mapping correspond to it. Since each QRAM operation costs $O(1)$ time, the QRAM update costs $O(N)$ time in total.

Next, we prove the B+ tree is perfectly balanced by induction. We only discuss the case that $N$ is not a power of $B$. Otherwise, the B+ tree is full, so it is obviously perfectly balanced. For a leaf node $u$, we can calculate the weight $w(u)$:
\begin{align*}
 w(u)&\geq\left\lfloor\frac{N}{\lceil N/B^h \rceil \cdot B^{h-1}}\right\rfloor
\geq \frac{N}{ (N/B^h+1)  \cdot B^{h-1}}-1\\
&=\frac{N}{N/B+ B^{h-1}}-1
>\frac{N}{N/B+ B^{\log_B N-1}}-1\\
&=\frac{N}{N/B+ N/B}-1
=B/2-1.
\end{align*}
Then, we know that a leaf node has a weight between $B/2$ and $B$ such that it is perfectly balanced. Consider a non-root node $u$ of height $h>0$, it must has $B$ perfectly balanced non-dummy children such that $w(u)\geq B\cdot B^h/2=B^{h+1}/2.$ Therefore, the B+ tree is perfectly balanced.
\vspace{-1mm}
\end{proof}

Then, we propose the hybrid quantum-classical range search algorithm on a static quantum B+ tree. We first introduce the quantum post-selection search in Section \ref{post}. The post-selection returns the answer to a range query efficiently when $\frac{k}{N}$ is large, where $N$ is the number of records for search and $k$ is the number of keys in the range. Obviously, we cannot assume $\frac{k}{N}$ is large, since the range query can return only one record, so we further proposed a hybrid quantum-classical range search algorithm to solve this problem. This algorithm contains two main steps: a global classical search and a local quantum search. In Section \ref{global}, we introduce the classical part. In Section \ref{local}, we introduce the quantum part based on a quantum post-selection. Then, we analyze the combination of the global classical search and the local quantum search in Section \ref{comb}.

\subsubsection{Quantum Post-Selection search}\label{post}
\leavevmode\\
\begin{figure}[htbp]
  \centering
  \subfigure{
  \includegraphics[width=0.7\columnwidth]{figure/post1.pdf}}
%\scalebox{1.0}{
%\Qcircuit @C=1.0em @R=0.2em @!R { \\
%	 	\nghost{{q}_{3} :  } & \lstick{{q}_{3} :  } & \gate{\mathrm{X}} & \ctrl{1} & \gate{\mathrm{X}} & \ctrl{1} & \qw & \qw & \qw\\
%	 	\nghost{{q}_{2} :  } & \lstick{{q}_{2} :  } & \gate{\mathrm{X}} & \ctrl{2} & \gate{\mathrm{X}} & \ctrl{2} & \qw & \qw & \qw\\
%	 	\nghost{{q}_{1} :  } & \lstick{{q}_{1} :  } & \qw & \qw & \qw & \qw & \qw & \qw & \qw\\
%	 	\nghost{{q}_{0}=\ket{} :  } & \lstick{{q}_{0} :  } & \qw & \gate{\mathrm{X}} & \qw & \gate{\mathrm{X}} & \meter & \qw & \qw\\
%	 	\nghost{\mathrm{{c} :  }} & \lstick{\mathrm{{c} :  }} & \lstick{/_{_{1}}} \cw & \cw & \cw & \cw & \dstick{_{_{\hspace{0.0em}0}}} \cw \ar @{<=} [-1,0] & \cw & \cw\\
%\\ }}
%$$v_i < 2$$
  \caption{Post-selection search for $QUERY(2, 5)$}
  \label{fig:postexp}
\end{figure}


To understand the quantum range search on a quantum B+ tree, we first discuss how to do an unstructured range search for $QUERY(x, y)$. Consider a QRAM $\mathcal{Q}$ such that $\mathcal{Q}\frac{1}{\sqrt{N}}\sum_{i=0}^{N-1}\ket{i}\ket{0}=\frac{1}{\sqrt{N}}\sum_{i=0}^{N-1}\ket{i}\ket{v_i},$ where $v_i$ is an integer value and $N$ is the number of values. Given $\mathcal{Q}$ and a pair of integers $x$ and $y$, we are to obtain the quantum states in the interval $[x, y]$ i.e., $\frac{1}{\sqrt{k}}\sum_{x\leq v_i\leq y}\ket{v_i},$ where $k$ is the number of values in the result. For simplicity, we use $\ket{in}=\frac{1}{\sqrt{k}}\sum_{x\leq v_i\leq y}\ket{v_i}$ to denote the values in the result and use $\ket{out}=\frac{1}{\sqrt{N-k}}\sum_{v_i < x \vee v_i > y}\ket{v_i}$ to denote the values not in the result. Then, we add an auxiliary qubit to obtain $$\frac{1}{\sqrt{N}}\sum_{i=0}^{N-1}\ket{v_i}\ket{0}=\frac{\sqrt{k}}{\sqrt{N}}\ket{in}\ket{0}+\frac{\sqrt{N-k}}{\sqrt{N}}\ket{out}\ket{0}.$$ Next, we need to change the quantum state from $\ket{0}$ to $\ket{1}$ after $\ket{out}$ by a quantum oracle $\mathcal{O}_{x,y}$:$$\ket{v_i}\ket{0} \rightarrow 
\left\{
	\begin{array}{ll}
		\ket{v_i}\ket{1} &\mbox{$v_i < x$ or $v_i > y$} ;\\
		\ket{v_i}\ket{0} &\mbox{otherwise} .\\
	\end{array}
\right.$$
Then, we obtain $\frac{\sqrt{k}}{\sqrt{N}}\ket{in}\ket{0}+\frac{\sqrt{N-k}}{\sqrt{N}}\ket{out}\ket{1}.$
The last step is to post-select the last qubit to be $\ket{0}$, which means we measure the last qubit, and if it is $1$, we repeat the whole process until it is $0$. After the post-selection, the state $\ket{out}$ is destroyed in the superposition so that we obtain $\ket{in}$. To analyze the complexity of the post-selection search, we obtain the following Lemma \ref{lemma1}.
\begin{lemma}\label{lemma1}
\vspace{-1mm}
	On average, the post-selection needs to be iterated $N/k$ times to obtain the answer to the range query, where $N$ is the total number of values and $k$ is the number of values in the query range.
	\vspace{-1mm}
\end{lemma}
\begin{proof}
After we measure the last auxiliary qubit, we will obtain $0$ with probability $\frac{k}{N}$ or $1$ with probability $\frac{N-k}{N}$ so that the expected number of measurements to obtain $0$ is $N/k$.
\vspace{-1mm}
\end{proof}
Figure \ref{fig:postexp} shows an example. Use $q_3q_2q_1$ to denote the binary representation of $v_i$ and use $q_0$ to denote the auxiliary qubit. Assume we have $\ket{q_3q_2q_1}=\frac{1}{2}(\ket{0}+\ket{1}+\ket{4}+\ket{7})$ and we are to answer $QUERY(2, 5)$ with post-selection. We add $q_0$ to the last, then apply the quantum circuit in Figure \ref{fig:postexp}. In the first dashed-line box, we consider the case $v_i<2$ such that we obtain $\ket{q_3q_2q_1}\ket{q_0}=\frac{1}{2}(\ket{0}+\ket{1})\ket{1}+\frac{1}{2}(\ket{4}+\ket{7})\ket{0}$. In the second dashed-line box, we consider the case $v_i>5$ such that we obtain $\ket{q_3q_2q_1}\ket{q_0}=\frac{1}{2}(\ket{0}+\ket{1}+\ket{7})\ket{1}+\frac{1}{2}\ket{4}\ket{0}$. Then, if we measure $q_0$ to be $0$ with probability $\frac{1}{4}$, then we can obtain $\ket{q_3q_2q_1}=\ket{4}$.

\subsubsection{Global Classical Search}\label{global}
\leavevmode\\
As described above, post-selection search costs $O(N/k)$ time, so it is obviously unacceptable to only use post-selection search to answer a range query. The reason is that if there is only one key-record pair in the query range, then $k=1$, which means the time complexity becomes $O(N)$. On the contrary, if $k$ is large, the post-selection search can be very fast. That is the reason why we use a data structure to do the range search even in a quantum computer.

Given a query $QUERY(x,y)$, in our quantum range search algorithm, the first step is to do a global classical search. The motivation of this step is to check if $k$ is large enough. We do the search levelwise starting from the root node. We call the nodes to be searched in a level the candidate nodes in the level. For example, the root node is the only candidate node in level $0$. Consider a candidate node $u$ in level $j$ has $f$ non-dummy children $c_0, c_1,\cdots, c_{f-1}$ and $f$ routing keys $(l_0,r_0), (l_1,r_1), \cdots, (l_{f-1},r_{f-1})$. For each $i\in [0, f-1]$, there are the following three cases.
\begin{itemize}
	\item Case 1: $r_i < x$ or $l_i > y$. That means $c_i$ does not have an answer. We do nothing.
	\item Case 2: $l_i < x$ and $x\leq r_i\leq y $ or $r_i > y$ and $x\leq l_i\leq y$. A part of the non-dummy key-record pairs below $c_i$ is in the answer, so add $c_i$ to the candidate nodes in level $j+1$. 
	\item Case 3: $l_i \geq x$ and $r_i \leq y$. That means all the non-dummy key-record pairs below $c_i$ are in the answer. Turn to a local quantum search starting from the candidate nodes in level $j$.
\end{itemize}

To analyze the complexity of the global classical search, we have the following Lemma \ref{lemma2}.

\begin{lemma}\label{lemma2}
\vspace{-1mm}
	The global classical search costs $O(\log_B N)$ time.
	\vspace{-1mm}
\end{lemma}
\begin{proof}
Assume in level $j$, the candidate nodes are $u_0, u_1, \cdots, u_{t-1}$, where $t\geq 3$ is the number of candidate nodes in the level. Obviously, all the key-record pairs below $u_1$ are in the answer, so we turn to the local quantum search in level $j-1$ and cannot reach level $j$, which makes a contradiction. Therefore, in each level, there are at most $2$ candidate nodes. Since the height of the tree is $O(\log_B N)$, there are totally $O(\log_B N)$ candidate nodes in the B+ tree. Hence, the global classical search costs $O(\log_B N)$ time.
\vspace{-1mm}
\end{proof}

For example, consider a query $QUERY(5, 11)$ given to the quantum B+ tree in Figure \ref{static}. We first check node 0. There is no child in Case 3. Node 1 and node 2 are candidate nodes since they are in Case 2. Then, we check node 1 and node 2. We find node 6 is a child in Case 3, so we turn to a local quantum search starting from node 1 and node 2.

\subsubsection{Local Quantum Search}\label{local}
\leavevmode\\
\begin{figure}[htbp]
  \centering
  \subfigure{
  \includegraphics[width=\columnwidth]{figure/local1.pdf}}
%\scalebox{1.0}{
%\Qcircuit @C=0.9em @R=0.2em @!R { \\
%	 	\nghost{\mbox{level-2 nodes} :  } & \lstick{\mbox{level-2 nodes} :  } & \qw & \lstick{/_{_{n_i}}}\qw & \qw & \multigate{2}{\mathrm{\mathcal{Q}_0}} & \qw & \qw & \qw & \qw & \qw \\
%	 	\nghost{\mbox{level-2 enumeration} :  } & \lstick{\mbox{level-2 enumeration} :  } & \qw & \lstick{/_{_{n_b}}}\qw & \gate{\mathrm{H}} & \ghost{\mathrm{\mathcal{Q}_0}} & \qw & \qw & \qw & \qw & \qw \\
%	 	\nghost{\mbox{level-3 nodes} :  } & \lstick{\mbox{level-3 nodes} :  } & \qw & \lstick{/_{_{n_i}}}\qw & \qw & \ghost{\mathrm{\mathcal{Q}_0}} & \qw & \qw & \multigate{3}{\mathrm{\mathcal{Q}_1}} & \qw & \qw \\
%	 	\nghost{\mbox{level-3 enumeration} :  } & \lstick{\mbox{level-3 enumeration} :  } & \qw & \lstick{/_{_{n_b}}}\qw & \qw & \qw & \qw & \gate{\mathrm{H}} & \ghost{\mathrm{\mathcal{Q}_1}} & \qw & \qw \\
%	 	\nghost{\mbox{keys} :  } & \lstick{\mbox{keys} :  } & \qw & \lstick{/_{_{n_k}}}\qw & \qw & \qw & \qw & \qw & \ghost{\mathrm{\mathcal{Q}_1}} & \gate{\mathrm{Post\mbox{-}Selection}} & \qw \\
%	 	\nghost{\mbox{records} :  } & \lstick{\mbox{records} :  } & \qw & \lstick{/_{_{n_r}}}\qw & \qw & \qw & \qw & \qw & \ghost{\mathrm{\mathcal{Q}_1}} & \qw & \qw \\
%\\ }}
  \caption{Local quantum search for $QUERY(5, 11)$}
  \label{fig:localexp}
\end{figure}

Since the local quantum search starts from at most two candidate nodes, consider answering $QUERY(x, y)$ starting from a node $u$ and another node $v$ as the candidate nodes in level $j$ and the height of the tree is $h$. Step 1 is to initialize the first $n_i$ quantum qubits to be $\frac{1}{\sqrt{2}}(\ket{u}+\ket{v}).$ Then, in Step 2, we add $n_b$ auxiliary qubits $\ket{0}$ to the last and also apply a Hadamard gate on each auxiliary qubit. We obtain $$\frac{1}{\sqrt{2}}(\ket{u}+\ket{v})\mathcal{H}\ket{0}\mathcal{H}\ket{0}\cdots \mathcal{H}\ket{0}=\frac{1}{\sqrt{2B}}(\ket{u}+\ket{v})\sum_{i=0}^{B-1}\ket{i}.$$ This step is to enumerate all the edges from the candidate nodes.
Then, in Step 3, we add $n_i$ qubits to the end and apply $\mathcal{Q}_0$ to obtain all the children of the candidate nodes, so we obtain $$\frac{1}{\sqrt{2B}}\ket{u}\sum_{i=0}^{B-1}\ket{i}\ket{c_i}+\frac{1}{\sqrt{2B}}\ket{v}\sum_{i=0}^{B-1}\ket{i}\ket{c_{i+B}},$$ where $c_0, \cdots, c_{B-1}$ are the $B$ children of $u$ and $c_B, \cdots, c_{2B-1}$ are the $B$ children of $v$. If we only look at the last $n$ qubits, we obtain $\frac{1}{\sqrt{2B}}\sum_{i=0}^{2B-1}\ket{c_i},$ which is the $2B$ children of $u$ and $v$. We repeat Step 2 and Step 3 for $h-j$ times so that we obtain all the $2B^{h-j}$ leaves below $u$ and $v$. Then, we do the same thing as Step 2 to enumerate all the $2B^{h-j+1}$ key-record pairs in the $2B^{h-j}$ leaves. In the last step, we apply $\mathcal{Q}_1$ to obtain all the key-record pairs below $u$ and $v$ and then do a post-selection search. Denote the $2B^{h-j+1}$ key-record pairs as $(key_0, rec_0), \cdots, (key_{2B^{h-j+1}-1}, rec_{2B^{h-j+1}-1})$. Then the quantum states become $\frac{1}{\sqrt{2B^{h-j+1}}}\sum_{i=0}^{2B^{h-j+1}-1}\ket{key_i}\ket{rec_i}.$ Similar to Section \ref{post}, we use $\ket{in}$ to denote the $k$ key-record pairs in the query range and use $\ket{out}$ to denote the other dummy key-record pairs and non-dummy key-record pairs which are not in the query range. We obtain $\frac{\sqrt{k}}{\sqrt{2B^{h-j+1}}}\ket{in}+\frac{\sqrt{2B^{h-j+1}-k}}{\sqrt{2B^{h-j+1}}}\ket{out}.$ If we do a post-selection, we can obtain $\ket{in}$ with probability $\frac{k}{2B^{h-j+1}}$. To analyze the complexity of a local quantum search, we have the following Lemma \ref{lemma3}.

\begin{lemma}\label{lemma3}
\vspace{-1mm}
	On average, the local quantum search needs $O(\log_B N)$ time.
	\vspace{-1mm}
\end{lemma}
\begin{proof}
By Lemma \ref{lemma1}, we repeat all the steps for $\frac{2B^{h-j+1}}{k}$ times on average. By the condition to trigger a local quantum search mentioned in Section \ref{global}, all the non-dummy key-record pairs below one of the children of $u$ and $v$ are all in the answer, therefore $k\geq \frac{1}{4}B^{h-j}$ by the definition of our quantum B+ tree. So, we need to repeat all the steps for at most $8B$ times, which is a constant time. In each iteration, we do Step 2 and Step 3 for at most $O(\log_B N)$ times, so the local quantum search needs $O(\log_B N)$ time.
\vspace{-1mm}
\end{proof}

For example, consider a query $QUERY(5, 11)$ on the quantum B+ tree in Figure \ref{static}. As mentioned in Section \ref{global}, the candidate nodes are node 1 and node 2. First, we initialize $\ket{\psi}=\frac{1}{\sqrt{2}}(\ket{1}+\ket{2})$. Then, we apply the quantum circuit in Figure \ref{fig:localexp}. After applying Hadamard gates and $\mathcal{Q}_0$, we obtain $\ket{\psi}=\frac{1}{\sqrt{8}}(\ket{4}+\ket{5}+\ket{6}+\ket{7}+\ket{8})+\frac{\sqrt{3}}{\sqrt{8}}\ket{dummy}$, which consists of all the children of node 1 and node 2. Then, after applying Hadamard gates and $\mathcal{Q}_1$, we obtain all the key-record pairs below node 1 and node 2, which is $\ket{\psi}=\frac{1}{\sqrt{32}}(\ket{1}\ket{rec_1}+\ket{2}\ket{rec_2}+\ket{4}\ket{rec_4}+\ket{6}\ket{rec_6}+\ket{8}\ket{rec_8}+\ket{10}\ket{rec_{10}}+\ket{13}\ket{rec_{13}}+\ket{16}\ket{rec_{16}}+\ket{19}\ket{rec_{19}}+\ket{21}\ket{rec_{21}})+\frac{\sqrt{22}}{\sqrt{32}}\ket{dummy}$. Finally, by a post-selection, we can obtain $\ket{\psi}=\frac{1}{\sqrt{3}}(\ket{6}\ket{rec_6}+\ket{8}\ket{rec_8}+\ket{10}\ket{rec_{10}})$ with probability $\frac{3}{32}$.

\subsubsection{Quantum Range Query}\label{comb}
\leavevmode\\
\begin{algorithm}[htbp]
\SetKwFunction{Query}{QUERY}
\SetKwFunction{Break}{break}
\caption{\protect\Query{x, y}} \label{alg-1}
\KwIn{a lower bound $x$ and an upper bound $y$.}
\KwOut{$\frac{1}{\sqrt{k}}\sum_{x\leq key_i \leq y}\ket{key_i}\ket{rec_i}$ where $k$ is the number of records with keys in $[x, y]$.}
	\tcp*[l]{A global classical search}
	Create lists $L$ and $L'$ to store candidate nodes;\\
	$L.add(root)$; \tcp*[r]{Initialize $L$ with the root node}
	$Found$ $\leftarrow$ $False$; \tcp*[r]{to denote if we need a quantum search}
	\While{$L$ consists of internal nodes}{
		$L'$ $\leftarrow$ $\emptyset$;\\
		\ForEach{node $u$ in $L$}{
			\ForEach{child $c_i$ of $u$}{
				\lIf{$l_i \geq x$ and $r_i \leq y$}{
					$Found$ $\leftarrow$ $True$; \Break ;
				}
				\lIf{$l_i \leq y$ and $r_i \geq x$}{
					$L'.add(c_i)$;
				}
			}
			\lIf{Found}{
				\Break ;
			}
		}
		\lIf{Found}{
			\Break ;
		}
		$L$ $\leftarrow$ $L'$;\\
	}
	\uIf{not Found}{
		$L'$ $\leftarrow$ $\emptyset$;\\
		\ForEach{node $u$ in $L$}{
			\ForEach{key-record pair $(key_i, rec_i)$ stored in $u$}{
				\lIf{$x \leq key_i \leq y$}{
					$L'.add((key_i, rec_i))$;
				}
			}
		}
		\Return{$\frac{1}{\sqrt{|L'|}}\sum \ket{L'_i}$}
	}
	\Else{
		\tcp*[l]{A local quantum search}
		$\ket{\psi}$ $\leftarrow$ $\frac{1}{\sqrt{|L|}}\sum \ket{L_i}$;\\
		\While{$\ket{\psi}$ consists of internal nodes}{
			$\ket{\psi}=\frac{1}{\sqrt{t}}\sum_{i=0}^{t-1}\ket{u_i}$ $\xmapsto{H-gates}$ $\frac{1}{\sqrt{tB}}\sum_{i=0}^{t-1}\ket{u_i}\sum_{j=0}^{B-1}\ket{j}$ $\xmapsto{\mathcal{Q}_0}$ $\frac{1}{\sqrt{tB}}\sum_{i=0}^{tB-1}\ket{c_i}$;\tcp*[r]{search for the children}
		}
		$\ket{\psi}=\frac{1}{\sqrt{t}}\sum_{i=0}^{t-1}\ket{u_i}$ $\xmapsto{H-gates}$ $\frac{1}{\sqrt{tB}}\sum_{i=0}^{t-1}\ket{u_i}\sum_{j=0}^{B-1}\ket{j}$ $\xmapsto{\mathcal{Q}_1}$ $\frac{1}{\sqrt{tB}}\sum_{i=0}^{tB-1}\ket{key_i}\ket{rec_i}$ $\xmapsto{\mbox{post-selection}}$ $\frac{1}{\sqrt{k}}\sum_{x\leq key_i\leq y}\ket{key_i}\ket{rec_i}$;\\
		\Return{$\frac{1}{\sqrt{k}}\sum_{x\leq key_i\leq y}\ket{key_i}\ket{rec_i}$}
	}
\end{algorithm}

In summary, we obtain Algorithm \ref{alg-1}. The quantum range query algorithm on a static quantum B+ tree works as follows. First, we do a global classical search in the classical part. We can obtain at most two candidate nodes. Then, we do a local quantum search in the quantum part starting from the two candidate nodes. In the local quantum search, we use the QRAM to obtain all the key-record pairs below the candidate nodes, then do a post-selection search to obtain the answer. To analyze the complexity of the algorithm, we have the following Theorem \ref{theo2}.
\begin{theorem}\label{theo2}
\vspace{-1mm}
	On average, the quantum range query algorithm returns the answer in $O(\log_B N)$ time.
\end{theorem}
\begin{proof}
By Lemma \ref{lemma2}, the global classical search needs $O(\log_B N)$ time.  By Lemma \ref{lemma3}, the local quantum search needs $O(\log_B N)$ time. Therefore, the quantum range query algorithm needs $O(\log_B N)$ time.
\vspace{-1mm}
\end{proof}
By Theorem \ref{theo2} and Theorem \ref{theostatic}, this algorithm is asymptotically optimal in a quantum computer.


\subsection{Dynamic Quantum B+ Tree}\label{dynamic}
In this section, we introduce how to make the static quantum B+ tree dynamic. In Section \ref{insert}, we introduce how to use the LSM-technique to make the quantum B+ tree support insertions. In Section \ref{delete}, we give a solution to perform deletions. In Section \ref{query}, we analyze the complexity of a range query in the dynamic version.

To use the quantum range query algorithm introduced in Section \ref{comb}, the quantum B+ tree needs to meet 3 requirements:
\begin{enumerate}
	\item Fanout limit: The fanout of each node should be at most $B$.
	\item Weight limit: The weight of each node of height $h$ should be at least $\frac{1}{4}B^{h+1}$.
	\item Level limit: All the leaves in a tree should be in the same level.
\end{enumerate}
The reason is that Lemma \ref{lemma3} is based on these 3 requirements. To the best of our knowledge, there is no existing data structure that meets our all requirements. For example, the original B+ tree \cite{comer1979ubiquitous} has no weight limit, and the original weight-balanced B+ tree \cite{arge1996optimal} has no fanout limit, since the fanout can be larger than $B$. The reason is that to meet the three requirements is meaningless in a classical computer. That is the motivation of us to make a new data structure that can work with our quantum range query algorithm.

\subsubsection{Insertion}\label{insert}
\leavevmode\\
We use the logarithmic method \cite{bentley1980decomposable} to make the quantum B+ tree support insertions. To store the key-record pairs, we build at most $\lfloor\log_B N\rfloor+1$ forests $F_0, \cdots, F_{\lfloor\log_B N\rfloor}$ where for each $i\in[0, \lfloor\log_B N\rfloor]$, the forest $F_i$ contains at most $B-1$ static quantum B+ trees of height $i$.

To perform an insertion like $INSERT(key, rec)$, we insert the key-record pair into a sorted list first. When the length of the sorted list reaches $B$, we flush it into $F_0$. Then, whenever a forest $F_i$ has $B$ quantum B+ trees, which means we have $B$ quantum B+ trees of height $i$, we merge the $B$ quantum B+ trees of height $i$ into a quantum B+ trees of height $i+1$, and add it into $F_{i+1}$. To analyze the complexity, we have the following Theorem \ref{theo3}.
\begin{theorem}\label{theo3}
\vspace{-1mm}
	The amortized cost of an insertion in a dynamic quantum B+ tree is $O(\log_B N)$.
\vspace{-1mm}
\end{theorem}
\begin{proof}
By Theorem \ref{theo1} in this paper and Theorem 3.1 in \cite{bentley1980decomposable}, $N$ insertions totally cost $O(N\log_B N)$ time. Therefore, the amortized cost of one insertion is $O(\log_B N)$.
\vspace{-1mm}
\end{proof}
Note that all quantum B+ trees have their classical parts and quantum parts. When doing insertions, any modification in the classical part has to be done in the quantum part to make the mappings in the QRAM correspond to the classical part. Since a QRAM operation costs $O(1)$ time as defined in Section \ref{QRAM}, Theorem \ref{theo3} also holds in the quantum part.

\subsubsection{Deletion}\label{delete}
\leavevmode\\

\begin{figure*}[tbp]
  \centering
  \subfigure[$DELETE(6, rec_6)$: Delete $(6, rec_6)$ in node 5. The weight of node 1 becomes $3$ which is less than $\frac{1}{4}B^2=4$, so node 1 becomes imbalanced. It borrows node 6 from node 2 such that node 1 and node 2 are both balanced.]{
    \label{fig:2-1}
    \includegraphics[width=0.54\textwidth]{figure/delete1.pdf}}
  \subfigure[$DELETE(27, rec_{27})$: Delete $(27, rec_{27})$ in node 9. Node 3 becomes imbalanced, and it cannot borrow node 8 from node 2. Node 2 and node 3 cannot be directly merged since they have 5 children, so the whole subtree is rebuilt.]{
    \label{fig:2-2}
    \includegraphics[width=0.44\textwidth]{figure/delete2.pdf}}
  \caption{Examples of deletions}
  \label{fig:deleteexp}
\end{figure*}

To perform a deletion like $DELETE(key, rec)$, we have two steps. The first step is to find the quantum B+ tree which contains the key-record pair. The second step is to delete the key-record pair in both the classical part and the quantum part of the quantum B+ tree. We then discuss these two steps one by one.

To locate the tree to do the deletion, we assign each key-record pair a unique ID in ascending order (e.g., by a counter). When doing an insertion $INSERT(key, rec)$, we assign the ID to the key-record pair, and maintain a B+ tree $T_0$ to store the one-to-one mapping from the key-record pair to its ID. When a key-record pair is inserted, we insert the key-record pair and its ID into $T_0$. When the key-record pair is deleted, we delete the key-record pair in $T_0$ accordingly. There is no other case to update $T_0$. Furthermore, we maintain another B+ tree $T_1$ to store the mapping from the key-record pair ID to the forest $F_i$ it belongs to. Similar to $T_0$, we do insertions and deletions in $T_1$ accordingly. In addition, when we merge $F_i$, we update $T_1$ for all the key-record pairs in $F_i$. To analyze the update cost in a merge, we have the following Lemma \ref{lemma4}.
\begin{lemma}\label{lemma4}
\vspace{-1mm}
	When merging $F_i$, the time complexity to update $T_1$ is $O(\log_B N)$.	\vspace{-1mm}
\end{lemma}
\begin{proof}
	Let $ID_l$ denote the least ID in $F_i$. For each $j<i$ and each key-record pair in $F_j$, the ID of the key-record pair is smaller than $ID_l$. Let $ID_r$ denote the greatest ID in $F_i$. Then, for each $j>i$ and each key-record pair in $F_j$, the ID of the key-record pair is greater than $ID_r$. Therefore, the update operations for the key-record pairs in $F_i$ can be merged into a range update. Then, we can use lazy propagation \cite{ibtehaz2021multidimensional} to do the range update in $O(\log_B N)$ time.
	\vspace{-1mm}
\end{proof}
By Lemma \ref{lemma4}, the extra cost to maintain $T_0$ and $T_1$ has no impact on Theorem \ref{theo3}, which means the amortized cost of insertion is still $O(\log_B N)$.

To delete the key-record pair in a B+ tree in $F_i$, we do a classical search to find the leaf that contains the key-record pair. Replace the key-record pair with a $dummy$. Then, check if its ancestors are still balanced. If an imbalanced ancestor is found, we first check if it can borrow a child from its sibling. Figure \ref{fig:2-1} shows an example in this case. If not, we check if it can be directly merged with its sibling, which means the node and its sibling have at most $B$ children. If not, we merge the node and its sibling by rebuilding the subtrees below them. Figure \ref{fig:2-2} shows an example in this case. Then, after rebalancing the B+ tree, we check if the root node still has at least two children. If not, we check if it can borrow a child from another B+ tree in $F_i$. If not, then if there are at least two B+ trees in $F_i$, we merge the root nodes of the two B+ trees. Otherwise, we remove the root node and downgrade the B+ tree from $F_i$ to $F_{i-1}$. 
\begin{theorem}\label{theo4}
\vspace{-1mm}
	The amortized cost of a deletion in a dynamic quantum B+ tree is $O(\log_B N)$.
\vspace{-1mm}
\end{theorem}
\begin{proof}
The first step costs $O(\log_B N)$ time, since it consists of two point queries in B+ trees.

Then consider the second step. Motivated by the analysis of partial rebuilding in \cite{overmars1983design}, we consider a node $u$ of height $h$ just after a rebuild. The node $u$ is perfectly balanced such that its weight $w(u)\geq \frac{1}{2}B^{h+1}$. Since it will become imbalanced if and only if $w(u)<\frac{1}{4}B^{h+1}$, there must be $\Omega(B^{h+1})$ deletions below the node $u$ or its siblings before that. So, it is charged $O(1)$ time for each deletion below it and its siblings. Then, for a deletion in a leaf node, each ancestor and its siblings are charged $O(1)$ time, so they are totally charged $O(\log_B N)$ time.

Therefore, the amortized cost of a deletion is $O(\log_B N)$.
\vspace{-1mm}
\end{proof}
Theorem \ref{theo4} shows that the complexity of deletion is the same as insertion, which is $O(\log_B N)$.

\subsubsection{Query}\label{query}
\leavevmode\\
To answer a query $QUERY(x,y)$, we do a global classical search and a local quantum search on $F_0, \cdots, F_{\lfloor\log_B N\rfloor}$. We initialize $\lfloor\log_B N\rfloor+1x$ lists $L_0,\cdots, L_{\lfloor\log_B N\rfloor}$. For each $i\in[0, \lfloor\log_B N\rfloor]$, we add the root nodes in $F_i$ into $L_i$. Then, we do the global classical search from $L_{\lfloor\log_B N\rfloor}$ to $L_0$. For $L_i$, we scan all the nodes in it one by one. Consider a node $u$ in $L_i$. We scan all $u$'s children. Similar to the algorithm in Section \ref{global}, if there is a child such that all the non-dummy key-record pairs are in the answer, then we turn to the local quantum search starting from $L_0,\cdots, L_i$. Otherwise, we add at most two children of $u$ into $L_{i-1}$, which may contain the answers. By Lemma \ref{lemma2}, since there are initially $O(\log_B N)$ quantum B+ trees, the classical global search costs $O(\log^2_B N)$ time.

Then, consider the local quantum search starting from $L_0,\cdots, L_i$. Consider the nodes $u_0, u_1,\cdots, u_{m-1}$ in the lists, where $m$ is the total number of nodes in $L_0,\cdots, L_i$. We initialize the quantum bits to be $\sum_{i=0}^{m-1}\frac{\sqrt{B^{h(u_i)+1}}}{\sqrt{\sum_{j=0}^{m-1} B^{h(u_j)+1}}}\ket{u_i},$ where $h(u_i)$ is the height of $u_i$, and $\frac{\sqrt{B^{h(u_i)+1}}}{\sqrt{\sum_{j=0}^{m-1} B^{h(u_j)+1}}}$ is the normalized amplitude of each $u_i$ such that each of the key-record pair below the nodes in the lists has the same amplitude in the result. By the amplitude encoding scheme in \cite{long2001efficient}, the initialization costs $O(m)$ time. Since by Lemma \ref{lemma2}, $m=O(\log_B N)$, the quantum bits can be obtained in $O(\log_B N)$ time. Then, we do the same Step 2 and Step 3 in Section \ref{local} to obtain the leaves below the nodes. Finally, we do a post-selection search as discussed in Section \ref{post}. To analyze the query cost, we have the following Theorem \ref{theo5}.
\begin{theorem}\label{theo5}
\vspace{-1mm}
	On average, the dynamic quantum B+ tree answers a range query in $O(\log^2_B N)$ time.
\vspace{-1mm}
\end{theorem}
\begin{proof}
As above mentioned, the global classical search costs $O(\log^2_B N)$ time. Consider the cost of the local quantum search. The initialization and the steps to obtain the leaves cost $O(\log_B N)$. Then, we multiply it by the average post-selection times. Let $N'$ denote the total number of key-record pairs below the nodes in $L_0,\cdots, L_i$. Then, by Lemma \ref{lemma1}, the post-selection needs to be iterated $O(N'/k)$ times on average. Since there are at most $2B\lfloor\log_B N\rfloor$ nodes in the lists and each node has a weight at most $B^{i+1}$, we have $N'\leq 2B^{i+2}\log_B N$. Before we turn to the local quantum search, we have found a child of a node in $L_i$ such that all the key-record pairs below the child are in the answer, such that $k\geq \frac{1}{4}B^i$. Therefore, $N'/k=O(\log_B N)$. Hence, the local quantum search costs $O(\log^2_B N)$ time on average.

Since both the global classical search and the local quantum search cost $O(\log_B^2 N)$ time, the dynamic quantum B+ tree answers a range query in $O(\log^2_B N)$ time on average.
\vspace{-1mm}
\end{proof}


\subsection{Static Quantum Range Tree}\label{range}

In this section, we show how to convert the classical range tree \cite{bentley1978decomposable} into a quantum data structure, as another extension of the static quantum B+ tree. Originally, the range tree answers a $d$-dimensional range query in $O(\log^d N+k)$ time. Using the quantum B+ tree, we can improve the complexity to $O(\log^d N)$. In the new problem, the key in a key-record pair is a $d$-dimensional vector $(key_0,\cdots,key_{d-1})$ where each $key_i$ is an integer, and in a query $QUERY(x, y)$, $x$ and $y$ are also two $d$-dimensional vectors, which are $(x_0,\cdots, x_{d-1})$ and $(y_0,\cdots, y_{d-1})$, respectively. The quantum range tree returns a superposition of all the key-record pairs such that for each $i\in[0, d-1]$, we have $x_i\leq key_i\leq y_i$.

We construct a static quantum range tree recursively. To build a $d$-dimensional quantum range tree, we first build a classical B+ tree indexing the $d$-th dimension of the keys. Then, we build a $d-1$-dimensional tree for each internal node in the B+ tree based on the key-record pairs below the internal node. Specifically, a $1$-dimensional quantum range tree is a static quantum B+ tree. Obviously, the space complexity and the time complexity of the construction are similar to the classical range tree.

Then, we discuss the $d$-dimensional static quantum range query. Starting from the $d$-th dimension, we search the B+ tree and find the $O(\log_B N)$ internal nodes in the search path which covers the $d$-th dimension of the query range. Then, turn to the quantum range trees on the $O(\log_B N)$ internal nodes and do a $d-1$-dimensional range search. Similar to the classical range tree, we then fetch the answers in $O(\log_B^{d-1} N)$ $1$-dimensional quantum range trees. By the same algorithm as described in Section \ref{comb}, we can obtain the key-record pairs within the query range in $O(O(\log_B^d N))$ time on average. The following Theorem \ref{theo6} shows the result.
\begin{theorem}\label{theo6}
\vspace{-1mm}
	On average, the quantum range tree answers a range query in $O(\log^d_B N)$ time.
\vspace{-1mm}
\end{theorem}
\begin{proof}
The first step is to recursively search the quantum range trees to obtain the $O(\log_B^{d-1} N)$ $1$-dimensional quantum range trees which contain answers. It costs $O(\log_B^{d-1} N)$ time. The second step is to perform a global classical search on the $O(\log_B^{d-1} N)$ quantum B+ tree. It costs $O(\log_B^d N)$ time. The third step is to perform a local quantum search starting from $O(\log_B^{d-1} N)$ candidate nodes returned in the second step. We first initialize the quantum bits in $O(\log_B^{d-1} N)$ time. Then, we do the same Step 2 and Step 3 in Section \ref{local} to obtain the leaves below the candidate nodes in $O(\log_B N)$ time. By Lemma \ref{lemma1}, we need to do a constant number of post-selections. Therefore, this step costs $O(\log_B^{d-1} N)$ time.

Therefore, the quantum range tree answers a range query in $O(\log^d_B N)$ time on average.
\vspace{-1mm}
\end{proof}











==> _old_sections/prev-conclusion.tex <==
\section{Conclusion}\label{sec:con}

In this paper, we study the quantum range query problem. We propose the static quantum B+ tree that answers a static quantum range query in $O(\log_B N)$ time, which is asymptotically optimal in quantum computers and exponentially faster than classical B+ trees. Furthermore, we extend it to a dynamic quantum B+ tree. The dynamic quantum B+ tree can support insertions and deletions in $O(\log_B N)$ time and answer a dynamic quantum range query in $O(\log^2_B N)$ time. We also discuss the high-dimensional static quantum range query. Based on the quantum B+ tree, we obtain a static quantum range tree which answers a $d$-dimensional static quantum range query in $O(\log^d_B N)$ time, which is also cannot be achieved by any classical algorithm. In the experiment, we did simulations to confirm the exponential speedup. We expect that the quantum data structures will show advantages in the real world.

In the future, we will study the following two questions. 
\begin{enumerate}
	\item Can we have a better index complexity in quantum data structures? To answer a range query, a dynamic quantum B+ tree needs $O(\log^2_B N)$ time and a quantum range tree needs $O(\log^d_B N)$ time. However, the classical data structures can answer a $1$-dimensional range query in $O(\log_B N + k)$ time \cite{comer1979ubiquitous} and answer a $d$-dimensional range query in $O(\log^{d-1} N + k)$ time \cite{chazelle1990lower}. Although the quantum data structures is exponentially faster than them, whether we could have the same index complexity as the best classical data structure is still an open problem.
	\item Can we answer a quantum query instead of classical queries? In our discussion, a query $QUERY(x, y)$ is given in classical bits. Consider a sequence of queries $QUERY(x_1, y_1), QUERY(x_2, y_2),$ $\cdots, QUERY(x_t, y_t)$. If the input is in quantum bits like $\frac{1}{\sqrt{t}}\sum_{i=1}^{t}$ $\ket{x_i}\ket{y_i},$ the classical queries becomes a quantum query. How to answer a quantum query is also an interesting question.
\end{enumerate}

==> _old_sections/prev-exp.tex <==
\section{Experiment}\label{exp}

\begin{figure}[htbp]
\vspace{-2mm}
  \centering
  \subfigure{
  \includegraphics[width=\columnwidth]{figure/legend1.eps}}
  \\
  \vspace{-4mm}
  \setcounter{subfigure}{0}
  \subfigure[Brightkite]{
    \label{fig:1-1}
    \includegraphics[width=0.48\columnwidth]{figure/Brightkite-1.eps}}
  \subfigure[Gowalla]{
    \label{fig:1-2}
    \includegraphics[width=0.48\columnwidth]{figure/Gowalla-1.eps}}
  \caption{Range queries with $d=1$ and $B=16$}
  \label{fig:1}
\end{figure}

\begin{figure}[htbp]
\vspace{-2mm}
  \centering
  \subfigure{
  \includegraphics[width=\columnwidth]{figure/legend2.eps}}
  \\
  \vspace{-4mm}
  \setcounter{subfigure}{0}
  \subfigure[Brightkite]{
    \label{fig:2-1}
    \includegraphics[width=0.48\columnwidth]{figure/Brightkite-2.eps}}
  \subfigure[Gowalla]{
    \label{fig:2-2}
    \includegraphics[width=0.48\columnwidth]{figure/Gowalla-2.eps}}
  \caption{Range queries with $d=2$ and $B=16$}
  \label{fig:2}
\end{figure}

\begin{figure*}[htbp]
\vspace{-2mm}
  \centering
  \subfigure{
  \includegraphics[width=0.6\textwidth]{figure/legend1.eps}}
  \\
  \vspace{-4mm}
  \setcounter{subfigure}{0}
  \subfigure[Brightkite]{
    \label{fig:3-1}
    \includegraphics[width=0.23\textwidth]{figure/Brightkite-1-s.eps}}
    \subfigure[Brightkite]{
    \label{fig:3-2}
    \includegraphics[width=0.23\textwidth]{figure/Brightkite-1-B.eps}}
  \subfigure[Gowalla]{
    \label{fig:3-3}
    \includegraphics[width=0.23\textwidth]{figure/Gowalla-1-s.eps}}
    \subfigure[Gowalla]{
    \label{fig:3-4}
    \includegraphics[width=0.23\textwidth]{figure/Gowalla-1-B.eps}}
  \caption{$1$-dimensional static range queries}
  \label{fig:3}
\end{figure*}

\begin{figure*}[htbp]
\vspace{-2mm}
  \centering
  \subfigure{
  \includegraphics[width=0.6\textwidth]{figure/legend2.eps}}
  \\
  \vspace{-4mm}
  \setcounter{subfigure}{0}
  \subfigure[Brightkite]{
    \label{fig:4-1}
    \includegraphics[width=0.23\textwidth]{figure/Brightkite-2-s.eps}}
    \subfigure[Brightkite]{
    \label{fig:4-2}
    \includegraphics[width=0.23\textwidth]{figure/Brightkite-2-B.eps}}
  \subfigure[Gowalla]{
    \label{fig:4-3}
    \includegraphics[width=0.23\textwidth]{figure/Gowalla-2-s.eps}}
    \subfigure[Gowalla]{
    \label{fig:4-4}
    \includegraphics[width=0.23\textwidth]{figure/Gowalla-2-B.eps}}
  \caption{$2$-dimensional static range queries}
  \label{fig:4}
\end{figure*}

\begin{figure*}[htbp]
\vspace{-2mm}
  \centering
  \subfigure{
  \includegraphics[width=0.6\textwidth]{figure/legend1.eps}}
  \\
  \vspace{-4mm}
  \setcounter{subfigure}{0}
  \subfigure[Brightkite]{
    \label{fig:5-1}
    \includegraphics[width=0.23\textwidth]{figure/Brightkite-i.eps}}
    \subfigure[Brightkite]{
    \label{fig:5-2}
    \includegraphics[width=0.23\textwidth]{figure/Gowalla-i.eps}}
  \subfigure[Gowalla]{
    \label{fig:5-3}
    \includegraphics[width=0.23\textwidth]{figure/Brightkite-q.eps}}
    \subfigure[Gowalla]{
    \label{fig:5-4}
    \includegraphics[width=0.23\textwidth]{figure/Gowalla-q.eps}}
  \caption{$1$-dimensional dynamic range queries}
  \label{fig:5}
\end{figure*}

In this section, we show some experimental results to further discuss the advantages of the quantum range query. The study of the real-world quantum supremacy \cite{arute2019quantum, boixo2018characterizing, terhal2018quantum}, which is to confirm that a quantum computer can do tasks faster than classical computers, is still a popular topic in the quantum area. We are not going to verify quantum supremacy in this problem, but we believe it will be verified in a future quantum computer. In this paper, we choose to evaluate the \emph{number of memory accesses} to make the comparisons, which corresponds to IOs in traditional searches. In the quantum data structures, a QRAM read operation is counted as 1 IO. In the classical data structures, a page access is counted as 1 IO. IOs cannot be regarded as the real execution time, since we have no any information about the real implementation of a QRAM, but they can reflect the potential of the data structures. In addition, the existing quantum simulators such as Qiskit \cite{wille2019ibm} and Cirq \cite{cirq} do not have a solution to simulate an efficient QRAM, so we choose to use C++ to perform the quantum simulations.

We conducted an experiment by simulating the quantum B+ tree on real-world datasets from SNAP \cite{leskovec2016snap}. The two datasets named Brightkite (4m) and Gowalla (6m) are two lists of check-ins with timestamps and locations. To compare the quantum B+ tree and the classical B+ tree, we took the timestamps as the $1$-dimensional data, which corresponds to the time-based range queries in real-world applications. We set the data size $N$ from $4096$ to $1048576$ and randomly generated $10000$ range queries. Figure \ref{fig:1} shows the result, where the x-axis $N$ denotes the number of records and the y-axis denotes the number of memory accessed needed to answer a range query on average. 

In addition, to show the advantage of the quantum range tree, we compared it with the classical range tree \cite{chazelle1990lower1}. Note that Chazalle \cite{chazelle1990lower1} has proved the lower bound of the orthogonal range searching problem, and the range tree is asymptotically optimal. We choose the state-of-the-art in the classical computer to make the comparison. We took the locations in the datasets as the $2$-dimensional data, which corresponds to the location-based range queries in real-world applications. Figure \ref{fig:2} shows the result. 

In Figure \ref{fig:1} and Figure \ref{fig:2}, we can learn that the cost of a classical range query grows linearly with $N$. The reason is that when the size of the dataset becomes larger, the size of the answer to a range query will also probably become larger. Compared to the classical competitors, the cost of a quantum range query only grows logarithmically with $N$, since it does not depend on the size of the answer. Based on these small datasets, the quantum range query is up to $1000\times$ faster than the classical query, which supports our claim in Section \ref{intro} that the quantum range query can be exponentially faster than the classical range query. 

Then, we study how the size of the answer and the block size affect the performance. Figure \ref{fig:3} shows the result in 1-dimension. First, we studied the performance with different selectivities (i.e., $\frac{k}{N}$). We varied the selectivity between $1\%$ and $10\%$ and the results are shown in Figure \ref{fig:3-1} and Figure \ref{fig:3-3}, where the x-axis denotes the selectivity and the y-axis denotes the number of memory accessed needed to answer a range query on average. We see that the IOs needed by the classical B+ tree grows linearly with $k$. However, the IOs needed by the quantum B+ tree even decreases. It seems surprising but in fact it is reasonable. The reason is that a larger $k$ shortened the process of the classical global search, such that we can turn to the local quantum search earlier. Also, as mentioned in Section \ref{post}, post-selection costs $O(N/k)$ time, so a larger $k$ also speedup the post-selection step. In addition, we studied how the block size affects the performance, and the results are shown in Figure \ref{fig:3-2} and Figure \ref{fig:3-4}, where the x-axis denotes the block size and the y-axis denotes the number of memory accessed needed to answer a range query on average. IOs needed by the classical B+ tree decreases fast, since with a larger $B$, fewer pages were accessed by the B+ tree. IOs needed by the quantum B+ tree increases, and this observation corresponds to a middle result in the proof of Lemma \ref{lemma3} that $B$ has an impact on the success rate of the post-selection step. 

Figure \ref{fig:4} shows the result in 2-dimension. We also varied the selectivity between $1\%$ and $10\%$, and varied $B$ from $4$ to $64$ to study their performance. The observations are almost the same as the $1$-dimensional cases. The only difference is that a larger $k$ did not lead to fewer IOs needed by the quantum range tree. The reason is that a larger $k$ leads to more candidate nodes for the subsequent local quantum search, which is different from the $1$-dimensional case.

The above is the result of static queries. We also conducted an experiment on the dynamic quantum B+ tree to study how the data insertion and deletion affect the efficiency of the quantum B+ tree. Following \cite{alsubaiee2014storage}, we insert all the records in the datasets with 1\% chance to delete an existing record instead of inserting a new record. $B$ is set to 16. Figure \ref{fig:5-1} and Figure \ref{fig:5-2} show the number of IOs needed to do the operation on average. We can learn that the dynamic quantum B+ tree needs $3$ times more IOs to insert or delete a record, since the data structure is more complex and it needs to do extra insertion in the QRAM. Figure \ref{fig:5-3} and Figure \ref{fig:5-4} show the number of memory accessed needed to answer a range query on a dynamic quantum B+ tree, where the selectivity is set to $5\%$. It is obvious that the dynamic quantum B+ tree has higher scalability since the IO cost increases much slower.

In conclusion, the quantum trees performs far better than the classical trees from the perspective of the number of memory accesses. In $1$-dimensional case, a larger $k$ and a smaller $B$ leads to a better performance. In $2$-dimensional case, a smaller $B$ leads to a better performance. Since the quantum B+ tree and the quantum range tree needs much fewer memory accesses to answer a range query, we conclude that they have the potential to outperform any classical data structure.






==> _old_sections/prev-intro.tex <==
\section{Introduction}\label{intro}
Consider a dataset of key-record pairs. The range query problem, which is to report all the key-record pairs with keys within a given range, has been widely used in many real-world applications. For example, a teacher may need to list all the students who obtained 40-60 marks in an exam, a smartphone buyer may need to list all the smartphones that sit around \$200-\$400, and a traveler may want to list all the nearby spots. 

Consider the scenario where a user named Alice wants to find an interesting movie. Each movie is described as a key-record pair where the key is the release date of the movie and the record is a feature vector which contains some attributes such as name, genre, and cast. Alice may want a movie of the 1990s. In the literature \cite{gupta2013location, covington2016deep}, we usually first find out all the movies from 1990 to 1999 as the candidates, and then give recommendations based on these candidates. The interval $[1990, 1999]$ given by Alice is the query range, where $1990$ is the lower bound and $1999$ is the upper bound. A range query returns all the movies with release dates within the query range. 

To answer range queries, many data structures \cite{bayer2002organization, comer1979ubiquitous, o1996log} have been proposed to store the key-record pairs. One representative data structure is the B+ tree. The B+ tree \cite{comer1979ubiquitous} is a widely-used existing data structure that answers a range query in $O(\log_B N +k)$ time, where $B$ is the branching factor of the B+ tree, $N$ is the total number of key-record pairs, and the output size $k$ is the number of records in the query range. Based on Yao's proof \cite{yao1981should}, it can be proved that the B+ tree is asymptotically optimal for range queries in classical computers. However, efficiency issues occur in quantum computers. Recently, quantum algorithms have attracted more and more attention. Many quantum algorithms \cite{shor1994algorithms, grover1996fast} have been proposed and are expected to show quadratic or even exponential speedup compared to classical algorithms, so many linear-complexity problems can be solved in sub-linear time in quantum computers. 
%For example, following \cite{campos2010simple}, consider using the KNN to give movie recommendations based on the candidates returned by a range query. Yue et al. \cite{ruan2017quantum} proposed a quantum KNN algorithm that only costs $O(d^3)$ time, where $d$ is the dimensionality of the feature vector. Since $k=O(N)$, the classical B+ tree answers a range query in $O(N)$ time in the worst case. 
Note that among existing methods, we need $O(\log_B N +k)$ time to do the range query, which is linear with the output size. This means that even if we can give recommendations in a sub-linear time with quantum algorithms \cite{ruan2017quantum, adhikary2020supervised, li2021vsql}, a linear time to generate the candidates is inevitable. Therefore, this linear-time range query will ruin all the advantages of the sublinear-time quantum algorithm. In fact, any classical range query algorithm has the same issue, which limits the potential of quantum algorithms in real-world applications.

Motivated by the serious limitations of the classical range query in quantum computers, we want to combine the advantages of data structures and quantum computation. Therefore, we propose the problem called the \emph{quantum range query}, which returns the answer in quantum bits. Specifically, the quantum range query $QUERY(x, y)$ does not return a list of key-record pairs, but returns quantum bits in a \emph{superposition} of all the key-record pairs with keys within the query range $[x, y]$, where the superposition is the ability of a quantum system to be in multiple states simultaneously. For example, consider a movie dataset $\{(key_0, rec_0), (key_1, rec_1),\cdots,$ $(key_{N-1}, rec_{N-1})\}$, where $N$ is the number of movies and each movie is described as a key-record pair as above mentioned. Assume that we can construct a data structure in the quantum computer to store all the key-record pairs. If Alice wants to obtain all the movies of the 1990s, a quantum range query $QUERY(1990, 1999)$ will search on the data structure and return quantum bits in a superposition of all the movies $(key_i, rec_i)$ whose $key_i$ is within the interval $[1990, 1999]$. Motivated by the different scenarios in real-world applications, we study the quantum range query problems in three different cases. The first case is that the dataset is immutable, so the problem is called the \emph{static quantum range query}. The second case is that insertions and deletions are supported in the dataset, and the problem is called the \emph{dynamic quantum range query}. The third case is that the keys in key-record pairs are high-dimensional points (e.g., the locations of restaurants), so the problem is called \emph{high-dimensional static quantum range query}.

The quantum range query problem has two distinctive characteristics. The first distinctive characteristic is that it allows the utilization of data structures, since existing quantum search algorithms do not use data structures. There are many quantum search algorithms \cite{grover1996fast, boyer1998tight, grover2005partial, durr1996quantum}, but all of them focused on the unstructured search, where the dataset is an unsorted list and the key-record pairs are not stored in a data structure. According to the study in \cite{boyer1998tight}, we can obtain a quantum range query algorithm which returns $k$ key-record pairs in $O(\sqrt{Nk})$ time. Although the cost of a range query grows sublinearly with $k$, this quantum range query algorithm cannot outperform its classical competitors such as the B+ tree. The main reason is that the existing quantum search algorithms do not take the advantage of data structures and they only discuss search problems in an unsorted list. However, the unstructured search hardly occurs in real-world applications. In the quantum range query problem, we allow to use a data structure to keep the dataset sorted.

The second distinctive characteristic is the use of quantum computation. Motivated by the quantum algorithms in other research fields, we have a question: Can we use the quantum techniques on the data structures to improve the complexity? The existing classical data structures \cite{bayer2002organization, comer1979ubiquitous, o1996log} are asymptotically optimal in classical computers, but there is a lot of room for improvement in quantum computers mentioned above. Since the number of quantum states increases exponentially with the increasing number of quantum bits, the quantum computer is supposed to help a lot of tasks. Quantum search should also be considered on data structures, but this topic has not been studied before.

Therefore, we first propose the \emph{static quantum B+ tree}, which is the first tree-like quantum data structure to our best knowledge. We choose the B+ tree \cite{comer1979ubiquitous} as the first data structure to study in quantum computers. Since the B+ tree is the most fundamental and widely-used data structure, it is considered the most suitable one to open a new world of quantum data structures. To take the full advantages of quantum parallelism, we design a hybrid quantum-classical algorithm to answer the static quantum range query. The hybrid design is very popular, especially in quantum machine learning \cite{kim2001batch}. According to \cite{abohashima2020classification}, many studies such as \cite{adhikary2020supervised, chakraborty2020hybrid, benedetti2019generative,schuld2019quantum,schuld2020circuit, ruan2017quantum, mitarai2018quantum} used hybrid quantum-classical algorithms to do machine learning, since this design can reduce the circuit depth (which signifies the total number of instructions in the quantum algorithm) so that high performance can be obtained. Specifically, the same B+ tree is stored both in a quantum computer and a classical computer. The classical component of the tree-building algorithm will bulk load the data and construct the B+ tree in a manner like \cite{kim2001batch}. We formally define the concept of a quantum memory in Section \ref{QRAM}, which is used to store mappings between bit-strings in a quantum computer. Each modification of the B+ tree in the classical computer will reflect in the quantum memory correspondingly. For example, if we add an edge from Node 2 to Node 3 in the B+ tree in the classical computer, we also add a mapping from 2 to 3 in the quantum memory. In the quantum computer, all the mappings from the nodes in the upper level to nodes in the lower level are maintained in the quantum memory. Our proposed quantum range query algorithm has the following two main steps.
\begin{enumerate}
	\item \emph{Global classical search}: The major goal is to find the candidate nodes in the B+ tree in the classical computer, where all the key-record pairs within the query range are stored under the candidate nodes, and at least $\frac{1}{8B}$ of the key-record pairs stored under these nodes are within the query range. It searches the B+ tree stored in the classical computer level by level, and returns a list of candidate nodes. Then, the candidate nodes will be passed to the local quantum search. This step will speedup the local quantum search, since to do the local quantum search from the candidate nodes has a lower circuit depth compared to search from the root node.
	\item \emph{Local quantum search}: The major goal is to obtain a superposition of all the key-record pairs within the query range under the candidate nodes. Starting from the candidate nodes, it searches the B+ tree stored in the quantum computer to access all the leaves under these tree nodes, and returns a superposition of all the key-record pairs under the candidate nodes. Since not all the key-record pairs in the superposition are within the query range, it then does a post-selection to obtain the superposition of the key-record pairs within the query range, and returns the superposition as the answer. This step makes the quantum range query more efficient than any classical range query due to quantum parallelism.
\end{enumerate}
We proved that a static quantum B+ tree answers a static quantum range query in $O(\log_B N)$ time and it is asymptotically optimal in quantum computers. The static quantum B+ tree achieves an exponential speedup compared to a classical B+ tree. We also discuss the dynamic quantum range query. The classical B+ tree accepts a key-record pair stored in the classical memory as the input of a insertion/deletion. By performing operations in the classical memory, this key-record pair is inserted/deleted. The same mechanism can be applied to a quantum B+ tree, but it is performed on the quantum memory (instead of the classical memory). A \emph{dynamic quantum B+ tree} accepts a key-record pair stored in the quantum memory, and performs operations in the quantum memory to insert/delete this key-record pair. During the insertion/deletion operation, the steps performed on the dynamic quantum B+ tree are conceptually the same as the steps performed on the classical B+ tree. Since a dynamic quantum B+ tree can perform insertions, deletions and range queries, it has all functionalities of a classical B+ tree, where the main difference is that the dynamic quantum B+ tree performs operations in the quantum memory and the classical B+ tree performs operations in the classical memory. For any key-record pair $(key, rec)$, we use $INSERT(key, rec)$ or $DELETE(key, rec)$ to insert or delete it in $O(\log_B N)$ time, and the complexity of a dynamic quantum range query is $O(\log^2_B N)$. Furthermore, we extend the quantum B+ tree to a $d$-dimensional static \emph{quantum range tree}, which answers a $d$-dimensional static quantum range query in $O(\log^d_B N)$ time.

%
%The quantum algorithm has been a widely discussed topic since Shor's algorithm was proposed in \cite{shor1994algorithms}, which can factor an integer $n$ in $O(polylog(n))$ time. This discovery showed the quantum algorithm can be theoretically exponentially faster than the most efficient classical algorithm in a non-trivial problem for the first time. It is believed that this algorithm can be used to break the RSA cryptosystem, which is widely used for data security. Encouraged by this discovery, many researchers studied other problems which quantum algorithms can solve more efficiently than classical algorithms. 
%
%Motivated by studies in other research field, we have a question: Can we use the quantum techniques on the tree data structures to improve the complexity? First we consider a point query, where the lower bound and the upper bound of the query range are the same. However, there is little hope to further improve the complexity of a point query. The membership problem is another problem that given a query key, we need to decide if the key exists in the data structure. Yao \cite{yao1981should} proved that for large key space, any cell-probe data structure need $\Omega(\log N)$ time to answer a membership problem in the worst case, where $N$ is the size of the data structure. Since a membership problem can be transformed into a point query, $\Omega(\log N)$ is also the lower bound on a tree data structure. In a quantum computer, this lower bound still holds. Ambainis \cite{ambainis1999better} proved an $\Omega(\log N)$ lower bound on quantum binary search, and claimed that quantum algorithms can only achieve a constant speedup over classical binary search. Based on this lower bound, Pranab et al. \cite{sen2001lower} further proved that the lower bound of static membership problem in the quantum cell-probe model is $\Omega(\log N)$, which means there is little hope that we can design a quantum data structure which can answer a point query much faster than classical data structures.
%
%In this paper, we focus on the range query. This kind of queries is very common in real world applications. For example, a teacher may need to list all the students who obtained 40-60 marks in an exam, a movie audience may need to list all the movies from 1995 to 2000, a smartphone buyer may need to list all the smartphones that sit around \$200-\$400, and a traveller may want to list all the nearby spots. Similar to a classical range query, a list of key-record pairs are stored in the data structure and a range query $QUERY(x, y)$ returns all the records with keys in the given range $[x, y]$. 
%
%Considering the above range query, we propose the first tree-like quantum data structure named the quantum B+ tree. We choose the B+ tree \cite{comer1979ubiquitous} as the first data structure to study in quantum computers. Since the B+ tree is the most fundamental and widely-used data structure, it is considered the most suitable one to open a new world of quantum data structures. Superposition is the ability of a quantum system to be in multiple states simultaneously For a given range $(x, y)$, we can use $QUERY(x, y)$ to obtain quantum bits (qubits) in a superposition of all the records with keys in the given query range. 
%
%To design the range query algorithm, we need to use the quantum RAM. Although the real-world practical implementation does not exist and the feasibility is still controversial \cite{ciliberto2018quantum}, different designs of a quantum RAM has been proposed such as \cite{park2019circuit, giovannetti2008quantum} and they have also been widely adopted in quantum algorithms such as \cite{kerenidis2019q, rebentrost2014quantum, wiebe2012quantum, kapoor2016quantum, wiebe2015quantum}, so we follow the same assumption that a quantum RAM can be implemented in the future. In this paper, we use the number of memory accesses to analyze the time complexity.
%
%To take the full advantages of quantum parallelism, we design a hybrid quantum-classical algorithm to answer the range query. The hybrid design is very popular especially in quantum machine learning. According to \cite{abohashima2020classification}, many studies such as \cite{adhikary2020supervised, chakraborty2020hybrid, benedetti2019generative,schuld2019quantum,schuld2020circuit, ruan2017quantum, mitarai2018quantum} used hybrid quantum-classical algorithms to do machine learning, since this design can reduce the circuit depth so that high performance can be obtained. Since the classical point query is as fast as the quantum range query, we need to first do a classical search, and when we confirm that the quantum search can do better than the classical search, we then change the process to a quantum search. To be more specific, the quantum range query algorithm has the following two main steps.
%\begin{enumerate}
%	\item Global classical search: We do a breadth-first search on the B+ tree to narrow the search range, where the search range is the range of all the tree nodes in the BFS queue. When we find that the ratio of the query range to the searchsearch range becomes high enough, we turn to the local quantum search;
%	\item Local quantum search: Starting from the tree nodes from the global classical search, we perform quantum operations to access to all the leaves below these tree nodes. Then, we do a post-selection to obtain the answer.
%\end{enumerate}
%This range query only costs $O(\log_B N)$ time, where $B$ is the branching factor and $N$ is the number of records. Note that the complexity of range query in a classical B+ tree is $O(\log_B N + k)$, where $k$ is the number of records with keys in the given range. Since $k=O(N)$ in the worst case, the quantum B+ tree achieves an exponential speedup. 
%
%When the query is a point query, since the global classical search will only maintain one tree node in the BFS queue, it will never turn to the local quantum search. Obviously, in that case, the $O(\log_B N)$ complexity holds since it is only a classical point query. When the query is a range query, we also prove that the time complexity is $O(\log_B N)$ with the local quantum search. Therefore, the quantum query algorithm is asymptotically optimal in quantum computers. Furthermore, we extend the $1$-dimensional quantum B+ tree to a $d$-dimensional quantum range tree, which can answer a $d$-dimensional range query in $O(\log^d_B N)$ time. We also discuss the dynamic quantum range query. A dynamic quantum B+ tree can perform classical insertions and deletions. For any key-record pair $(key, rec)$, we can use $INSERT(key, rec)$ or $DELETE(key, rec)$ to insert or delete it in $O(\log_B N)$ time, and it slowers the complexity of a dynamic quantum range query to $O(\log^2_B N)$. 
%
%Since the number of quantum states increases exponentially when the number of quantum bits increases linearly, the quantum computer is supposed to be more powerful to help a lot of calculations. In this paper, we also use this advantage to improve the complexity. However, there is a difference between the classical range query and the quantum range query in the output. Instead of returning a list of all the answers, a quantum range query returns quantum bits. The result is a superposition of all the key-record pairs in the answer. Unlike the classical answer, if we measure the quantum bits, we can only randomly get one of the key-record pair, and then the superposition will be collapsed. Although quantum range query cannot return a classical list of all the answers, we still consider it very meaningful, since we do not regard the result as a final output available to a user but an input to other quantum algorithms. The motivations of the quantum range query can be concluded as the following:
%\begin{itemize}
%	\item It can speedup quantum model training with label binning. Studies such as \cite{dougherty1995supervised, xue2017efficient, berg2021deep} claimed that the label binning before model training can improve the accuracy in classification tasks. The authors concluded that choices of different label binning strategies affect the training convergence, and it is difficult to select them without any parameter search. Assume we need to train a quantum model such as \cite{gambs2008quantum, adhikary2020supervised} which use single-shot training with the input of a superposition of all the data with the same label, we can do a quantum range query $QUERY(x, y)$ where $x$ and $y$ are the boundaries of the label bin, and use the output as the training data. If we use a classical B+ tree, we need to use $O(\log_B N+k)$ time to select all the records in the label bin, where $k$ is the number of records binned in the same label. The quantum range query returns the input to the quantum model in $O(\log_B N)$ time, which is exponentially faster.
%	\item It can speedup the range filter in a recommendation system. For example, a recommendation system like \cite{gupta2013location, covington2016deep} usually has two steps. The first step is to select a small part of the all the items as the candidates. The second step is to use a model (e.g., a neural network) to predict the scores of the items for a user. Assume the model prediction costs $O(T)$ time for an item and the first step is a range filter (e.g., to choose the locations of restaurants), the total recommendation process costs $O(\log^2_B N+k+kT)$ time. In a quantum computer, we can use a quantum range query to select the candidates, and use a quantum model to predict the scores. This process costs $O(\log^2_B N +T)$ time, which is a lot faster than its classical competitor. Another example is the time-periodic-biased KNN \cite{campos2010simple}, which is to select the records produced in the same month but different years and use KNN for movie recommendation. On average, the calculation will cost $O(\log_B N + N/12)$ time since the range query returns $N/12$ records on average. With a quantum range query, we can select the records in $O(\log_B N)$ time. Then, with the $O(d^3)$ quantum KNN algorithm \cite{ruan2017quantum} where $d$ is the dimension of the record, the whole process only costs $O(\log_B N + d^3)$, which is exponentially faster than the classical competitor if $d<<N$.
%	\item We believe that more quantum algorithms will be benefitted in the future. Since quantum algorithms always receives quantum data as the input, we think that it is very common that quantum algorithms return answers in a superposition. For example, the HHL algorithm \cite{harrow2009quantum} returns the answer to a linear system of equations in a superposition, and it becomes a subroutine of the quantum SVM \cite{rebentrost2014quantum}.
%\end{itemize}
%
%After the design and the analysis, we also conduct an experiment to verify the correctness of the quantum range query algorithms. We compare the classical trees and the quantum trees on two real-world datasets. To be more specific, we compare classical B+ trees and quantum B+ trees on $1$-dimensional datasets, and also compare classical range trees and quantum range trees on $2$-dimensional datasets. We use the number of memory accesses to evaluate the execution time and show that a quantum range query does exponentially fewer memory accesses to obtain the answer. The experimental results confirm the exponential speedup of the quantum range queries.

To the best of our knowledge, we are the first to study the quantum range query problem, and we are the first to propose a tree-like quantum data structure. We consider that the first tree-like quantum data structure will open a new world of quantum data structures. Unlike the classical range query, a quantum range query returns answers in quantum bits. We consider the quantum output very useful, and discuss the real-world utilization in Section \ref{application}. In summary, our contributions are shown in the following:
\begin{itemize}
	\item We are the first to study the quantum range query problems.
	\item We are the first to propose a quantum tree-like data structure, which is the quantum B+ tree.
	\item We design a hybrid quantum-classical algorithm that can answer a range query on a static quantum B+ tree in $O(log_B N)$ time, which does not depend on the output size and is asymptotically optimal in quantum computers.
	\item We further make the static quantum B+ tree support insertions and deletions in $O(\log_B N)$ time, and the complexity of the range query becomes $O(\log^2_B N)$.
	\item We extend the static quantum B+ tree to the static quantum range tree, which answers a $d$-dimensional static range query in $O(\log^d_B N)$ time. 
	\item We conducted the experiment to confirm the exponential speedup of the quantum range queries on real-world datasets. We considered both time-based range query and location-based range query, which is the widely used in real-world applications. In the experiment, the quantum range query is up to $1000\times$ faster than a classical range query.
\end{itemize}


The rest of the paper is organized as follows. In Section \ref{pre}, we introduce some basic knowledge used in this paper about quantum algorithms. In Section \ref{related}, we introduce related work. In Section \ref{problem}, we define the problem and further discuss the problem.  In Section \ref{alg}, we show the design of a quantum B+ tree. In Section \ref{exp}, we do simulations to show the efficiency and correctness of our algorithms. In Section \ref{con}, we give a conclusion.


==> _old_sections/prev-preliminary.tex <==
\section{Preliminaries}\label{pre}

The bit is a basic unit when we want to store data in the memory or on disks. The bit in classical computers usually has two \emph{states}, which are $0$ and $1$. In a quantum computer, we also have the bit, which is called the \emph{quantum bit}. For simplicity, we use \emph{qubit} in the following. Similar to the bit in a classical computer, the qubit also has states. To describe the states of a qubit, we usually use the \emph{Dirac notation} \cite{dirac1939new, bayer2002organization} which looks like $\ket \cdot$. We can write an integer in it to denote a \emph{basis state}, or write a symbol in it to denote a \emph{mixed state}, where the symbol can be regarded as the name of the qubit or qubits. For example, $\ket 0$ and $\ket 1$ are two \emph{basis states} of a qubit, which correspond to the state 0 and state 1 of a classical bit, respectively. Different from the classical bit, the state of a qubit can be `between' $\ket 0$ and $\ket 1$. If we use $q$ to name this single qubit, then we can use $\ket q$ to denote such a \emph{mixed state} of it. We can express the mixed state with a linear combination of the two basis states:
$\ket q = \alpha \ket 0 + \beta \ket 1.$
$\alpha$ and $\beta$ are two complex numbers, which are usually called the \emph{amplitudes}. We have $|\alpha|^2 + |\beta|^2=1$, where $|\alpha|^2$ means the absolute square of $\alpha$. Like reading a classical bit, we can measure a qubit. The measurement will collapse the superposition of the qubit so that we can only obtain the result state 0 with probability $|\alpha|^2$ or state 1 with probability $|\beta|^2$. For example, there is a qubit $q$ with the mixed state 
$$\ket q = (0.36+0.48i) \ket 0 + (0.48-0.64i) \ket 1.$$
If we measure this qubit, we can obtain 0 with probability $|0.36+0.48i|^2=0.36^2+0.48^2=0.36$ or 1 with probability $|0.48-0.64i|^2=0.48^2+0.64^2=0.64$. Since the probability should sum to 1, $|0.36+0.48i|^2+|0.48-0.64i|^2=1$ holds.

Considering that there are two basis states of a qubit, if we have two qubits, the basis states will become $\ket{00}$, $\ket{01}$, $\ket{10}$ and $\ket{11}$. If we measure a qubit, the measurement will change the state of another qubit. Such a phenomenon is called \emph{quantum entanglement} \cite{schrodinger1935discussion}. For example, assume that there are two qubits $q_0$ and $q_1$, which combines a \emph{quantum register} $\psi$:
\begin{align*}
\ket{\psi}=\ket{q_1 q_0} &= \frac{1}{\sqrt{2}}\ket 0(0.6 \ket 0 + 0.8 \ket 1)+\frac{1}{\sqrt{2}}\ket 1(\frac{1}{\sqrt{2}}\ket 0+\frac{1}{\sqrt{2}}\ket 1)\\
%&= \frac{0.6}{\sqrt{2}}\ket{00} + \frac{0.8}{\sqrt{2}}\ket{01} + \frac{1}{2}\ket{10} + \frac{1}{2}\ket{11}\\
&= \frac{0.6}{\sqrt{2}}\ket{0} + \frac{0.8}{\sqrt{2}}\ket{1} + \frac{1}{2}\ket{2} + \frac{1}{2}\ket{3},
\end{align*}
where $\ket{q_1} = \frac{1}{\sqrt{2}}\ket 0 + \frac{1}{\sqrt{2}}\ket 1$ is expressed outside the parentheses, and $\ket{q_0}$ is expressed in the parentheses and depends on \ket{q_1} due to the \emph{quantum entanglement}. If we measure $q_1$, we will obtain 0 or 1 with probability 0.5. If we obtain 0, the state of $q_0$ will be changed to $\ket{q_0}=0.6 \ket 0 + 0.8 \ket 1$. Otherwise, the state of $q_0$ will be changed to $\ket{q_0}=\frac{1}{\sqrt{2}}\ket 0+\frac{1}{\sqrt{2}}\ket 1$. Therefore, the measurement of $q_1$ will change the state of $q_0$, so these two entangled qubits have $4$ basis states $\ket{00}, \ket{01}, \ket{10}, \ket{11}$ with amplitudes $\frac{0.6}{\sqrt{2}}, \frac{0.8}{\sqrt{2}}, \frac{1}{2}, \frac{1}{2}$, respectively. Similarly, we can extend this system to $n$ qubits $q_{n-1}, q_{n-2}, \cdots q_0$ and they have $2^n$ basis states and corresponding $2^n$ amplitudes.

Similar to the classical computer, we also have wires and gates in quantum computers. The wire starting at the left hand side and ending at the right hand size denotes a timeline, representing the process from an earlier moment to a later moment. The gates in quantum computers are called \emph{quantum gates}, which are used to transform the states of qubits. For example, \emph{Hadamard gate} \cite{hadamard1893resolution, nielsen2001quantum} is a very useful quantum gate, which turns $\ket 0$ into $\frac{1}{\sqrt{2}}\ket 0 + \frac{1}{\sqrt{2}}\ket 1$ and turns $\ket 1$ into $\frac{1}{\sqrt{2}}\ket 0 - \frac{1}{\sqrt{2}}\ket 1$. The following shows an example of the visualization of a quantum circuit which consists of a qubit (denoted by $q$), a classical register (denoted by $c$), a Hadamard gate (denoted by the box containing an H), and a measurement (denoted by an icon like a real meter). 
\begin{center}
	\scalebox{0.9}{
\Qcircuit @C=1.0em @R=1.0em @!R { 
	 	\nghost{{q} :  } & \lstick{{q} :  } & \gate{\mathrm{H}} & \meter & \qw & \qw\\
	 	\nghost{{c} :  } & \lstick{{c} :  } & \lstick{/_{_{1}}} \cw & \dstick{_{_{\hspace{0.0em}0}}} \cw \ar @{<=} [-1,0] & \cw & \cw\\
}
\hspace{5mm}
}
\vspace{1mm}
\end{center}
As above mentioned, $q$ is the qubit. The \emph{single-line wire} is a timeline, which denotes the order of the quantum gates coming to the qubit. The \emph{double-line wire} denotes the classical register. The small number below the double-line wire after $/$ is the number of bits in the classical register, so the classical register has $1$ bit in this example. Since there is a small number $0$ under the down arrow from the meter icon, the $0$-th bit in the classical register $c$ stores the result of the measurement. 

Here, a Hadamard gate can be represented by the Dirac notation:
$$\ket 0 \rightarrow \frac{1}{\sqrt{2}}\ket 0 + \frac{1}{\sqrt{2}}\ket 1; \ket 1 \rightarrow \frac{1}{\sqrt{2}}\ket 0 - \frac{1}{\sqrt{2}}\ket 1, $$ where the two cases of the quantum transformation are separated by ``;'', ``$\rightarrow$'' denotes the quantum transformation of a Hadamard gate, the quantum states before the transformation is on the left of ``$\rightarrow$'' and the quantum states after the transformation is on the right of ``$\rightarrow$''.
For example, assume an input $\ket{q}=\frac{1}{\sqrt{2}}\ket{0}+\frac{1}{\sqrt{2}}\ket{1}$. The Hadamard gate turns $\ket 0$ into $\frac{1}{\sqrt{2}}\ket 0 + \frac{1}{\sqrt{2}}\ket 1$ and turns $\ket 1$ into $\frac{1}{\sqrt{2}}\ket 0 - \frac{1}{\sqrt{2}}\ket 1$, so the quantum bit will become $$\ket{q}=\frac{1}{\sqrt{2}}(\frac{1}{\sqrt{2}}\ket 0 + \frac{1}{\sqrt{2}}\ket 1)+\frac{1}{\sqrt{2}}(\frac{1}{\sqrt{2}}\ket 0 - \frac{1}{\sqrt{2}}\ket 1)=\ket{0}.$$ If we measure the result, we obtain 0.

Similar to the classical computer, the gates in the quantum computer can be applied on multiple qubits. The following quantum circuit shows an example. 
\begin{center}
	\scalebox{0.8}{
\Qcircuit @C=1.0em @R=1.0em @!R { 
	 	\nghost{{q}_{1} :  } & \lstick{{q}_{1} :  } & \gate{\mathrm{X}} & \ctrl{1} & \meter & \qw & \qw & \qw\\
	 	\nghost{{q}_{0} :  } & \lstick{{q}_{0} :  } & \qw & \gate{\mathrm{X}} & \qw & \meter & \qw & \qw\\
	 	\nghost{\mathrm{{c} :  }} & \lstick{\mathrm{{c} :  }} & \lstick{/_{_{2}}} \cw & \cw & \dstick{_{_{\hspace{0.0em}1}}} \cw \ar @{<=} [-2,0] & \dstick{_{_{\hspace{0.0em}0}}} \cw \ar @{<=} [-1,0] & \cw & \cw
}
\hspace{5mm}
}
\vspace{1mm}
\end{center}
We have two qubits $q_0$ and $q_1$ in this example. We apply an \emph{$X$-gate} \cite{nielsen2001quantum} (also known as a NOT-gate) on $q_1$ (denoted by the box containing X with only one wire as input from the left), and a \emph{controlled-$X$} gate on both $q_0$ and $q_1$ (denoted by the box containing X with one wire as input from the left (i.e., $\ket{q_0}$) and another wire as input from the top (i.e., $\ket{q_1}$ after the $X$-gate)). Although an $X$-gate and a controlled-$X$ gate use the same symbol X, they could be differentiated by their different numbers of input wires. The $X$-gate is to swap the amplitudes of $\ket 0$ and $\ket 1$. We can represent it by the Dirac notation: $\ket 0 \rightarrow \ket 1; \ket 1 \rightarrow \ket 0$. 
The controlled-$X$ gate has two parts: $q_1$ is the \emph{control} qubit since it is in the wire from the top, and $q_0$ is the \emph{target} qubit since it is in the wire from the left. The controlled-$X$ gate applies an $X$-gate on the target qubit if the control qubit is $\ket 1$; otherwise, keep the target qubit unchanged. We can represent it by the Dirac notation: $\ket 0\ket{q_0}\rightarrow \ket 0\ket{q_0}; \ket 1\ket{q_0}\rightarrow \ket 1 X \ket{q_0}$, where ``$X \ket{q_0}$'' denotes applying an $X$-gate on $q_0$. In the programming language, we can express this operation as: If $q_1=1$, then $q_0 = \mbox{NOT } q_0$. Consider the following three examples of input:
\begin{enumerate}
	\item $\ket{q_1q_0}=\ket{00}$. After the $X$-gate on $q_1$, $\ket{q_1q_0}=\ket{10}$. Since $\ket{q_1}=\ket{1}$, apply an $X$-gate on $q_0$, so the result is $\ket{11}$.
	\item $\ket{q_1q_0}=\ket{11}$. After the $X$-gate on $q_1$, $\ket{q_1q_0}=\ket{01}$. Since $\ket{q_1}=\ket{0}$, do nothing, so the result is $\ket{01}$.
	\item $\ket{q_1q_0}=\frac{1}{\sqrt{2}}\ket{00}+\frac{1}{\sqrt{2}}\ket{11}$. After the $X$-gate on $q_1$, $\ket{q_1q_0}=\frac{1}{\sqrt{2}}\ket{10}+\frac{1}{\sqrt{2}}\ket{01}$. The result is $\frac{1}{\sqrt{2}}\ket{11}+\frac{1}{\sqrt{2}}\ket{01}.$
\end{enumerate}


Usually, we describe such a quantum transformation consisting of a series of quantum gates as a \emph{quantum oracle}. A quantum oracle can be regarded as a black box of a quantum circuit which we focus on the quantum operation it can perform but do not need to know the quantum circuit in detail. The concept of the quantum oracle has been widely used in many studies such as \cite{grover1996fast, shor1994algorithms, wiebe2015quantum, zhang2018quantum}. Since different gate sets (which represent instruction sets in classical computers) may cause different time complexities and the general quantum computer is still at a very early stage, we usually use the query complexity to study quantum algorithms, which is to measure the number of queries to the quantum oracles. In the quantum algorithm area, many studies such as \cite{li2021sublinear, kapralov2020fast, montanaro2017quantum, naya2020optimal, hosoyamada2018quantum, li2019sublinear, kieferova2021quantum} assume that quantum oracles costs $O(1)$ time, and analyze the time complexity based on this assumption. We also follow this common assumption in this paper.



==> _old_sections/prev-problem.tex <==
\section{Problem Definition}\label{problem}

In this section, we formally define the quantum range query problems and further discuss them. 

Consider an immutable dataset $D=\{(key_0, rec_0), (key_1, rec_1),$ $\cdots, (key_{N-1}, rec_{N-1})\}$ where $key_i$ is an integer stored in $n_k$ bits, $rec_i$ is a bit-string record stored in $n_r$ bits, and $(key_i, rec_i)$ is a key-record pair for each $i\in [0, N-1]$, we need to answer a range query in quantum bits. Note that in our discussion, the keys are integers, but they can be extended to real numbers easily. A range query is expressed as $QUERY(x, y)$ where $x$ is the lower bound and $y$ is the upper bound. A classical range query returns a list of key-record pairs whose keys are in the query range. The returned list $\{(key_{l_0}, rec_{l_0}),\cdots, (key_{l_{k-1}}, rec_{l_{k-1}})\}$ is a subset of $D$, where $k$ is the length of the list, $l_i$ is the index of the key-record pair in $D$ for each $i\in [0, k-1]$, and $x\leq key_{l_i}\leq y$ holds for each $i\in [0, k-1]$. A quantum range query returns a superposition of all the key-record pairs in the list. We have the following Definition \ref{defstatic}.
\begin{definition}[Static Quantum Range Query]\label{defstatic}
\vspace{-1mm}
	Given an immutable dataset $D=\{(key_0, rec_0), (key_1, rec_1), \cdots, (key_{N-1},$ $rec_{N-1})\}$, a quantum range query $QUERY(x, y)$ is to return the quantum state $$QUERY(x, y)=\frac{1}{\sqrt{k}}\sum_{i=0}^{k-1}\ket{key_{l_i}}\ket{rec_{l_i}},$$ where for each $i\in [0, k-1]$, $x\leq key_{l_i} \leq y$.
	\vspace{-1mm}
\end{definition}
To discuss the lower bound of the static quantum range query problem, we introduce another problem. The membership problem is another problem that given a query key, we need to decide if the key exists in the data structure. Ambainis \cite{ambainis1999better} proved an $\Omega(\log N)$ lower bound on quantum binary search, and claimed that quantum algorithms can only achieve a constant speedup over classical binary search. Based on this lower bound, Pranab et al. \cite{sen2001lower} further proved that the lower bound of the static membership problem in the quantum cell-probe model is $\Omega(\log N)$. Then, we have the following Theorem \ref{theostatic}.

\begin{theorem}\label{theostatic}
\vspace{-1mm}
The time complexity to answer a static quantum range query is $\Omega(\log N)$.
\vspace{-1mm}
\end{theorem}
\begin{proof}
Consider a static quantum range query $QUERY(x, x)$, it answers whether the key $x$ exists in the dataset, so it answers a static membership problem. By \cite{sen2001lower}, the time complexity to answer a static membership problem in quantum computers is $\Omega(\log N)$. Therefore, the time complexity to answer a static quantum range query is also $\Omega(\log N)$.
\vspace{-1mm}
\end{proof}

Then, consider the dynamic case. Insertions and deletions are supported in the dynamic range query. An insertion $INSERT(key, rec)$ inserts the key-record pair $(key, rec)$ into the dataset, so we obtain a new dataset $D\cup \{(key, rec)\}$. A deletion $DELETE(key, rec)$ deletes the key-record pair $(key, rec)$ from the dataset, so we obtain a new dataset $D\setminus \{(key, rec)\}$. We have the following Definition \ref{defdynamic}.

\begin{definition}[Dynamic Quantum Range Query]\label{defdynamic}
\vspace{-1mm}
	Given a dynamic dataset $D=\{(key_0, rec_0), (key_1, rec_1), \cdots, (key_{N-1},$ $rec_{N-1})\}$ which supports insertions and deletions, a quantum range query $QUERY(x, y)$ is to return the quantum state $$QUERY(x, y)=\frac{1}{\sqrt{k}}\sum_{i=0}^{k-1}\ket{key_{l_i}}\ket{rec_{l_i}},$$ where for each $i\in [0, k-1]$, $x\leq key_{l_i} \leq y$.
\vspace{-1mm}
\end{definition}

In the high-dimensional cases, the keys in the dataset are not integers but $d$-dimensional vectors. For each $i\in [0, N-1]$, $key_i$ consists of $d$ integers $(key_{i, 0}, key_{i, 1}, \cdots, key_{i, d-1})$. Correspondingly, $x$ and $y$ in a range query $QUERY(x, y)$ are two $d$-dimensional vectors, where $x=(x_0, x_1,\cdots, x_{d-1})$ and $y=(y_0, y_1,\cdots, y_{d-1})$. Then, we have the following Definition \ref{defhigh}.

\begin{definition}[High-Dimensional Static Quantum Range Query]\label{defhigh}
\vspace{-1mm}
	Given an immutable dataset $D=\{(key_0, rec_0), (key_1, rec_1), \cdots, (key_{N-1},$ $rec_{N-1})\}$ where the keys are $d$-dimensional vectors, a quantum range query $QUERY(x, y)$ is to return the quantum state $$QUERY(x, y)=\frac{1}{\sqrt{k}}\sum_{i=0}^{k-1}\ket{key_{l_i}}\ket{rec_{l_i}},$$ where for each $i\in [0, k-1]$ and $j\in [0, d-1]$, $x_j\leq key_{l_i, j} \leq y_j$.
\vspace{-1mm}
\end{definition}

To further discuss the problems, we introduce the quantum random access memory (QRAM) in Section \ref{QRAM}, since the QRAM should be used to store the dataset in quantum computers. In Section \ref{application}, we introduce several applications of the results of quantum range queries. Instead of returning a list of all the answers, a quantum range query returns quantum bits. The result is a superposition of all the key-record pairs with keys within the query range. Unlike the classical answer, if we measure the quantum bits, we can only randomly get one of the key-record pairs, and then the superposition will be collapsed. Although quantum range query cannot return a classical list of all the answers, we still consider it very meaningful, since we do not regard the result as a final output available to a user but as an input to other quantum algorithms. Therefore, we list several applications to show how to use the quantum range query results in future real-world applications.
  
 
\subsection{Quantum Random Access Memory}\label{QRAM}

Following \cite{kerenidis2017quantum, saeedi2019quantum}, in this paper, we assume a classical-write quantum-read QRAM. It takes $O(1)$ time to store a classical record. Also, it takes $O(1)$ time to accept a superposition of addresses and return a superposition of the corresponding records. The main difference from a classical memory is that we assume that it takes $O(1)$ time to read multiple records. Therefore, we have the following Definition \ref{def:QRAM}.

\begin{definition}[Quantum Random Access Memory (QRAM)]\label{def:QRAM}
A QRAM $\mathcal{Q}$ is an ideal model which performs store and load operations in $O(1)$ time. 
\begin{itemize}
	\item A store operation: $\mathcal{Q}[address]=value$, where $value$ is a bit-string;
	\item A load operation: $$\mathcal{Q}\frac{1}{\sqrt{k}}\sum_{i=0}^{k-1}\ket{address_i}\ket{x}=\frac{1}{\sqrt{k}}\sum_{i=0}^{k-1}\ket{address_i}\ket{x\oplus value_i},$$ where $k$ is the number of required values, $x$ is the initial value of the destination register to store the results of the load operation, and $\oplus$ denotes the XOR operation.
\end{itemize}
\end{definition}

Assume there is a QRAM $\mathcal{Q}$, then $\mathcal{Q}$ needs to support two operations. The first operation is to store classical data. An operation $\mathcal{Q}[address]=value$ will store a classical value at the specified address in $O(1)$ time, where $address$ and $value$ are two bit-strings. In this operation, we can regard $\mathcal{Q}$ as an array $A$ in a classical computer, where $A(i)$ is the value stored in the $i$-th entry and $i$ is the address. For simplicity, we also use $\mathcal{Q}[address]$ to denote the value stored at the address. The second operation is to load quantum data. In this operation, $\mathcal{Q}$ works as a quantum mapping from the addresses to the values: $\mathcal{Q}\ket{address}\ket{x}=\ket{address}\ket{x\oplus value}$, where $\oplus$ denotes the XOR operation and $\ket x$ is the initial state of the returned qubits. Furthermore, the loading operation $$\mathcal{Q}\frac{1}{\sqrt{k}}\sum_{i=0}^{k-1}\ket{address_i}\ket{0}=\frac{1}{\sqrt{k}}\sum_{i=0}^{k-1}\ket{address_i}\ket{A(address_i)}$$ costs $O(1)$ time, where $k$ is the number of required values. The load and store operation cost $O(1)$ time is a basic assumption in the database area when we calculate the complexity. In the quantum algorithm area, this quantum mapping can be regarded as a quantum oracle, and many studies such as \cite{li2021sublinear, kapralov2020fast, montanaro2017quantum, naya2020optimal, hosoyamada2018quantum, li2019sublinear, kieferova2021quantum} also assume the quantum oracle costs $O(1)$ time.

The concept of a QRAM has been widely adopted in many quantum algorithms \cite{kerenidis2019q, rebentrost2014quantum, wiebe2012quantum, kapoor2016quantum, wiebe2015quantum}. Since many quantum algorithms were proposed to have a sub-linear time complexity compared to their linear classical competitors, if a linear time is needed to load the data, they may lose the advantage. Note that even with the assumption of QRAMs, the quantum range query is still non-trivial. The reason is that the QRAM only maps the addresses to values, but to fetch all the addresses we need is a non-trivial task. Considering there is no existing quantum data structure, if we use quantum algorithms with a QRAM and without any data structure, we can use quantum counting \cite{brassard1998quantum} to estimate the number of answers $k$ in $O(\sqrt{N})$ time, then use the unstructured quantum search \cite{boyer1998tight} to find the answers in $O(\sqrt{Nk})$ time. The search can even be slower than a classical data structure search. 

%Consider the Grover's algorithm \cite{grover1996fast} introduced in Section \ref{related}. If we want to use Grover's algorithm as a common database search algorithm, we need a quantum random access memory (QRAM) to store all the records. Assume the query is to find the position of the word ``unicorn'' in \emph{The Witcher} and the word only appears once in the book. If all the $N$ words are stored in the QRAM, then the QRAM can do the following quantum operation efficiently: $$\frac{1}{\sqrt{N}}\sum_{i=0}^{N-1}\ket{i}\ket{0}\rightarrow \frac{1}{\sqrt{N}}\sum_{i=0}^{N-1}\ket{i}\ket{word_i},$$where $N$ is the total number of words in the book and $word_i$ is the $i$-th word in the book. Then, we can build a quantum oracle that flips the amplitude of $\ket{i}$ if $word_i$ is ``unicorn''. With this oracle, we can find the position of the word in $O(\sqrt{N})$ time. Besides this application of Grover's algorithm, many other quantum algorithms \cite{kerenidis2019q, rebentrost2014quantum, wiebe2012quantum, kapoor2016quantum, wiebe2015quantum} also use the concept of a QRAM. Since many quantum algorithms were proposed to have a sub-linear time complexity compared to their linear classical competitors, if a linear time is needed to load the data, they may lose the advantage. It is believed that the QRAM can load data more efficiently, so it becomes an important concept in quantum algorithms.

%There are mainly two kinds of designs of a QRAM: the bucket-brigade QRAM (BB-QRAM) \cite{giovannetti2008quantum} and the flip-flop QRAM (FF-QRAM) \cite{park2019circuit}. In a BB-QRAM, a qutrit is used as a switch in the architecture to tell the signal to go left or go right in the next level. The qutrit is a three-level quantum system which is defined to have three states: $\ket{left}$, $\ket{right}$ and $\ket{wait}$. Since the qutrits in the state $\ket{wait}$ are regarded as inactive qutrits, there are only $O(\log N)$ active qutrits for one memory access. Therefore, the BB-QRAM saves physical resources and energy compared to the fanout QRAM \cite{nielsen2001quantum}. The FF-QRAM is a circuit-based QRAM, which could be used in the state preparation step of a quantum algorithm. The FF-QRAM can encode the data into not only the basis state but also the amplitudes. After the circuit of a FF-QRAM, a quantum database will be generated and it can be the input of other quantum algorithms. 

%Although there are existing designs of QRAMs like the bucket-brigade QRAM  \cite{giovannetti2008quantum} and the flip-flop QRAM \cite{park2019circuit}, scalable and workable implementation of a QRAM has not been achieved yet. In fact, the feasibility of the QRAM is also controversial \cite{ciliberto2018quantum}. However, we believe it is a problem that can be solved in the future. Following \cite{kerenidis2017quantum, saeedi2019quantum}, in this paper, we assume a classical-write quantum-read QRAM. It takes $O(1)$ time to store a classical record. Also, it takes $O(1)$ time to accept a superposition of addresses and return a superposition of the corresponding records just like the above example. 
%
%Assume there is a QRAM $\mathcal{Q}$, then $\mathcal{Q}$ needs to support two operations. The first operation is to store classical data. An operation $\mathcal{Q}[address]=value$ will store a classical value at the specified address in $O(1)$ time, where $address$ and $value$ are two integers. In this operation, we can regard $\mathcal{Q}$ as an array $A$ in a classical computer, where $A(i)$ is the value stored in the $i$-th entry and $i$ is the address. For simplicity, we also use $\mathcal{Q}[address]$ to denote the value stored at the address. The second operation is to load quantum data. In this operation, $\mathcal{Q}$ works as a quantum mapping from the addresses to the values: $\mathcal{Q}\ket{address}\ket{x}=\ket{address}\ket{x\oplus value}$, where $\oplus$ denotes the XOR operation and $\ket x$ is the initial state of the returned qubits. Furthermore, the loading operation $$\mathcal{Q}\frac{1}{\sqrt{k}}\sum_{i=0}^{k-1}\ket{address_i}\ket{0}=\frac{1}{\sqrt{k}}\sum_{i=0}^{k-1}\ket{address_i}\ket{A(address_i)}$$ costs $O(1)$ time, where $k$ is the number of required values. The load and store operation cost $O(1)$ time is a basic assumption in the database area when we calculate the complexity. In the quantum algorithm area, this quantum mapping can be regarded as a quantum oracle, and many studies such as \cite{li2021sublinear, kapralov2020fast, montanaro2017quantum, naya2020optimal, hosoyamada2018quantum, li2019sublinear, kieferova2021quantum} also assume the quantum oracle costs $O(1)$ time.
% 
% Note that even with the assumption of QRAMs, the quantum range query is still non-trivial. The reason is that the QRAM only maps the addresses to values, but to fetch all the addresses we need is a non-trivial task. Considering there is no existing quantum data structure, if we use quantum algorithms with a QRAM and without any data structure, we can use quantum counting \cite{brassard1998quantum} to estimate the number of answers $k$ in $O(\sqrt{N})$ time, then use the unstructured quantum search \cite{boyer1998tight} to find the answers in $O(\sqrt{Nk})$ time. The search can even be slower than a classical data structure search. 
%
\subsection{Application of Quantum Range Query}\label{application}

In this section, we introduce how to use the result of a quantum range query in future real-world applications. We discuss several real-world applications where other quantum algorithms can be benefitted from the quantum range query.

The first application is for label binning in quantum machine learning. Assume there is a classification task with a training dataset $\{(x_1, y_1),\cdots,$ $(x_N, y_N)\}$ where for each $i\in[1,N]$, $x_i$ is the feature vector and $y_N$ is a continues label. There are many studies showing that packing labels into bins can improve the accuracy of the label prediction. In \cite{dougherty1995supervised}, Dougherty et.al. introduced equal-width binning, which is to bin the labels into $k$ equal-sized bins, where $k$ is a user parameter. They conducted experiments on 16 datasets to show that the label binning can improve the accuracy of Naive Bayes. In \cite{xue2017efficient}, Xue et.al. used equal-size binning to bin the labels into $k$ bins. They conducted experiments to show that label binning can improve the accuracy of SVM and the best performance is obtained when the bin size is set to $O(N^{1/3})$. They pointed out that $k$ will affect the quality of the result. In \cite{berg2021deep}, Berg et.al. used a neural network to do image classification. They did three tasks: Age estimation, head pose estimation, and historical image dating. In the experiment, two tasks were improved by label binning. They also claimed that $k$ has an impact on the prediction performance, and it is difficult to select $k$ for a given problem without an extensive parameter search. 

The above studies are based on classical machine learning. We can learn that many machine learning algorithms can be improved by label binning in some scenarios, so it is reasonable to consider it may also improve the accuracy of quantum machine learning algorithms. For example, to train a quantum model, there is an existing method called single-shot training \cite{adhikary2020supervised}. To train a classical model, we input $(x_i, y_i)$ one by one and $N$ iterations are needed in an epoch. In single-shot training, we generate a superposition of all the $x_i$ with the same label $y_i$ and input the data in one iteration, so an epoch contains only $k$ iterations, where $k$ is the number of bins. To obtain such a superposition, we can make a quantum range query of the bin boundaries to generate the superposition, which should be exponentially faster than existing methods like \cite{long2001efficient} to encode the data in a bin into quantum bits one by one.
%
%, it takes $O(N/k)$ time. By a range query to a quantum B+ tree, we only need $O(\log_B N)$ time.

The second application is for a range filter of a recommendation system. For example, a recommendation system \cite{gupta2013location, covington2016deep} usually has two steps. The first step is to select a small part of all the items as the candidates. The second step is to use a prediction model (e.g., a neural network) to predict the scores of the items for a user. For example, assume that we want the system to recommend us a movie from 1990 to 1999. Now we have a model \cite{biancalana2011context} to predict the score of the movie for a user. The first step is to select all the $k$ movies from 1990 to 1999 from the database with $N$ movies to obtain $\{movie_1, movie_2,\cdots,movie_k\}$, which costs $O(\log N + k)$ time . The second step is that for each $movie_i$, we use the model to predict the score $s(movie_i)$ for a recommendation.  Assume the model prediction costs $T$ time for a movie, then it totally costs $O(kT)$ time. Therefore, the classical recommendation system costs $O(\log N + k + kT)$ time. Now consider a quantum system for the movie recommendation. Assume that all the movies have been stored in a quantum data structure, and we can obtain the $k$ movies in quantum bits by a quantum range query in $O(\log_B N)$ time: $$QUERY(1990, 1999)=\frac{1}{\sqrt{k}}\sum_{i=0}^{k-1}\ket{i}\ket{movie_i}.$$ Then, with a quantum model, we can predict the score of all the movies in $T$ time: $$\frac{1}{\sqrt{k}}\sum_{i=0}^{k-1}\ket{i}\ket{movie_i}\ket{0}\rightarrow \frac{1}{\sqrt{k}}\sum_{i=0}^{k-1}\ket{i}\ket{movie_i}\ket{s(movie_i)}.$$ Therefore, the quantum recommendation system only needs $O($ $\log_B N +T)$ time. A multi-dimensional example is the location-based restaurant recommendation \cite{gupta2013location}. We can use a high-dimensional quantum range query to obtain a speedup.

Another example is the time-periodic-biased KNN. Campos et.al. \cite{campos2010simple} studied how to use KNN to do movie recommendations. They found that it can improve the accuracy to only consider the rating datasets from the last month before the recommendation time in different years.  That means they need to select the records produced in the same month but in different years. Given a B+ tree containing all the movies sorted by the dates in the year, the calculation costs $O(\log_B N + N/12)$ time since the range query returns $N/12$ records on average. Assume that we can use a quantum range query to select the $N/12$ records in $O(\log_B N)$ time. Note that there is an existing $O(d^3)$ quantum KNN algorithm \cite{ruan2017quantum} where $d$ is the dimension of the feature vector. Therefore, the whole process only costs $O(\log_B N + d^3)$. In most cases, $d$ is much smaller than $N$. Assuming $d=O(\log N)$, we can find that the quantum time-periodic-biased KNN is exponentially faster than its classical competitor.
 
Besides the above applications, we believe that more and more quantum algorithms will be benefitted in the future. Since quantum algorithms always receive quantum data as the input, we think it is very common that quantum algorithms return answers in a superposition. For example, the HHL algorithm \cite{harrow2009quantum} returns the answer to a linear system of equations in a superposition, and it becomes a subroutine of the quantum SVM \cite{rebentrost2014quantum}. Specifically, in the database area, we consider the future quantum top-$k$ algorithms and query optimization will be benifitted by quantum data structures, for which a quantum B+ tree can preprocess data to narrow the searching space.
 

==> _old_sections/prev-related.tex <==
\section{Related Work}\label{sec:related}

The classical range query problem has been studied for decades but it is not such a popular topic now. The reason is that a lot of different data structures have been proposed to solve this problem in different scenarios and there is very little room for further significant improvement. 

For the static range query and the dynamic range query, the B-tree \cite{bayer2002organization} and the B+ tree \cite{comer1979ubiquitous} are widely-used. The B+ tree is a tree data structure which can find a key in $O(\log_B N)$ time, where $N$ is the number of key-record pairs and $B$ is the branching factor. Then, $O(k)$ time is needed to load the $k$ key-record pairs in the query range, so the range query on a B+ tree costs $O(\log_B N + k)$ time. The membership problem is another problem that given a query key, we need to decide if the key exists in the data structure. Yao \cite{yao1981should} proved that for a large key space, any cell-probe data structure needs $\Omega(\log N)$ time to answer a membership problem in the worst case, where $N$ is the size of the data structure. Since a membership problem can be transformed into a point query, $\Omega(\log N)$ is also the lower bound on a tree data structure, so the B+ tree is asymptotically optimal for range queries in classical computers.

For the high-dimensional static range query, Bentley \cite{bentley1978decomposable} proposed the range tree to answer it in $O(\log^d N + k)$ time, where $d$ is the dimension of the keys. In addition, the range tree needs $O(N\log^{d-1} N)$ storage space. Then, Chazelle further improved the complexity. Chazelle \cite{chazelle1990lower1, chazelle1990lower2} proposed the lower bounds for the $d$-dimensional cases: $O(k+polylog(N))$ time complexity with $\Omega(N(\log N/\log$ $\log N)^{d-1}))$ storage space and $\Omega((\log N/$ $\log (2C/N))^{d-1}+k)$ time complexity with $C$ units storage space where the lower bound of query I/O cost is provably tight for $C=\Omega(N(\log N)^{d-1})$. 

However, all the above classical data structures have the same problem: The execution time grows linearly with $k$, which makes them useless for quantum algorithms. For example, the $O(\log N)$ quantum algorithm for linear systems of equations \cite{harrow2009quantum}, the $O(\sqrt{N})$ quantum Bayesian inference algorithm \cite{low2014quantum}, and the $O(\log N)$ quantum support vector machine \cite{rebentrost2014quantum} are all sub-linear time algorithms. If a linear time is needed to load the data, the advantages of sub-linear time algorithms will disappear. So, the data structures in quantum computers for range queries should be considered.

The quantum database searching problem is also very popular in the quantum algorithm field. Grover's algorithm is described as a database search algorithm in \cite{grover1996fast}. It solves the problem of searching a marked record in an unstructured list, which means that all the $N$ records are arranged in random order. On average, the classical algorithm needs to perform $N/2$ queries to a function $f$ which tells us if the record is marked. More formally, for each index $i$, $f(i)=1$ means the $i$-th record is marked and $f(i)=0$ means the $i$-th record is unmarked. Note that only one record is marked in the database. If we have a quantum circuit to calculate this function, then we can build a Grover oracle $G:\ket{x} \rightarrow (-1)^{f(x)}\ket{x}$. Taking the advantage of quantum parallelism, Grover's algorithm can find the index of the marked record with $O(\sqrt{N})$ queries to the oracle. The main idea is to first ``flip" the amplitude of the answer state and then reduce the amplitudes of the other states. One such iteration will enlarge the amplitude of the answer state and $O(\sqrt{N})$ iterations should be performed until the probability that the qubits are measured to be the answer comes close to 1. Then, an improved Grover's algorithm was proposed in \cite{boyer1998tight}. We are also given the function $f$ to mark the record, but $k$ records are marked at this time. The improved Grover's algorithm can find one of the $k$ marked records in $O(\sqrt{N/k})$ time. If we make the function $f$ to mark the records with keys within a query range, then this algorithm returns one of the $k$ key-record pairs in $O(\sqrt{N/k})$ time, and it needs $O(\sqrt{Nk})$ time to answer a range query. 

The execution time of the quantum database search algorithm grows linearly with the square root of $k$, which is better than the classical data structures. However, the time complexity is even worse than the classical structures. Due to this observation, although Grover described the Grover's algorithm as a database search algorithm in \cite{grover1996fast}, we do not consider it capable of real-world database searching. The main reason is that in most real-world scenario, the database is not unstructured. Thus, the data structure should be considered in real-world databases. 

In the database area, there are also plenty of studies discussing how to use quantum computers to further improve traditional database queries. For example, \cite{uotila2022synergy, schonberger2022applicability, fankhauser2021multiple, trummer2015multiple} discussed quantum query optimization, which is to use quantum algorithms like quantum annealing \cite{finnila1994quantum} to optimize a traditional database query. However, compared with the quantum range query discussed in this paper, the existing studies are in a different direction. The existing studies are discussing how to use a quantum algorithm to optimize range queries in a classical computer, where the query returns a list of records. In this paper, we discuss how to use a classical algorithm to optimize range queries in a quantum computer, where the query returns quantum bits in a superposition of records. We focus on a quantum data structure stored in a quantum computer, where the classical algorithm is only to assist the query. To our best knowledge, in the database area, we are the first to discuss quantum algorithms in this direction.

In conclusion, the existing classical data structures and the existing quantum database searching algorithms cannot solve the range query problem in quantum computers perfectly.

%We assume the readers have the basic knowledge of the classical data structures such as B-trees \cite{bayer2002organization}, B+ trees \cite{comer1979ubiquitous} and range trees \cite{bentley1978decomposable}. The quantum random access memory (QRAM) is a basic assumption in this paper, since the quantum B+ tree is stored in the QRAM. In Section \ref{QRAM}, we introduce the quantum random access memory. In Section \ref{application}, we introduce some related works which could be benefited by the quantum B+ tree. 
%
%\subsection{Quantum Random Access Memory}\label{QRAM}
%
%Grover's algorithm is described as a database search algorithm in \cite{grover1996fast}. It solves the problem of searching a record in an unstructured list, which means that all the $N$ records are arranged in random order. On average, the classical algorithm needs to perform $N/2$ queries to a function $f$ which tells us if the record is the answer. More formally, for each index $x$, $f(x)=1$ means the record is the answer and $f(x)=0$ means the record is not an answer. If we have a quantum circuit to calculate this function, then we can build a Grover oracle $G:\ket{x} \rightarrow (-1)^{f(x)}\ket{x}$. Taking the advantage of quantum parallelism, Grover's algorithm can find the index of the answer with $O(\sqrt{N})$ queries to the oracle. The main idea is to first ``flip" the amplitude of the answer state and then reduce the amplitudes of the other states. One such iteration will enlarge the amplitude of the answer state and $O(\sqrt{N})$ iterations should be performed until the probability that the qubits are measured to be the answer comes close to 1. Grover mentioned in \cite{grover2005partial} that the database is supplied in the form of a quantum oracle. In fact, the Grover oracle also contains the information of the query condition, but not only a database. This oracle can recognize the solution and Grover's algorithm is from ``recognizing the solution'' to ``knowing the solution'' \cite{nielsen2001quantum}, so Grover's algorithm has limitations in database searching. For example, the generation of the Grover oracle can be even slower than classical search \cite{seidel2021automatic}, since we need to linearly scan the database to load the data into quantum bits. However, many algorithms such as \cite{durr1996quantum, wiebe2015quantum} invoke Grover's algorithm as a subroutine due to its quadratic speedup compared to classical algorithms.
%
%If we want to use Grover's algorithm as a common database search algorithm, we need a quantum random access memory (QRAM) to store all the data. Assume the query is to find the position of the word ``unicorn'' in \emph{The Witcher} and the word only appear once in the book. If all the words are stored in the QRAM, then the QRAM can do the following quantum operation efficienly: $$\frac{1}{\sqrt{N}}\sum_{i=0}^{N-1}\ket{i}\ket{0}\rightarrow \frac{1}{\sqrt{N}}\sum_{i=0}^{N-1}\ket{i}\ket{word_i},$$where $N$ is the total number of words in the book and $word_i$ is the $i$-th word in the book. Then, we can build a quantum oracle which flips the amplitude of $\ket{i}$ if $word_i$ is ``unicorn''. With this oracle, we can find the position of the word in $O(\sqrt{N})$ time. Besides this application in Grover's algorithm, many other quantum algorithms \cite{kerenidis2019q, rebentrost2014quantum, wiebe2012quantum, kapoor2016quantum, wiebe2015quantum} also use the concept of a QRAM. Since many quantum algorithms were proposed to have a sub-linear time complexity compared to their linear classical competitors, if we still need linear time to load the data, they may lose the advantage. That is why the concept of QRAM is important in this area, since it is believed that the QRAM can load data more efficiently.
%
%There are mainly two kinds of designs of a QRAM: the bucket-brigade QRAM (BB-QRAM) \cite{giovannetti2008quantum} and the flip-flop QRAM (FF-QRAM) \cite{park2019circuit}. In a BB-QRAM, a qutrit is used as a switch in the architecture to tell the signal to go left or go right in the next level. The qutrit is a three-level quantum system which is defined to have three states: $\ket{left}$, $\ket{right}$ and $\ket{wait}$. Since the qutrits in the state $\ket{wait}$ are regarded as inactive qutrits, there are only $O(\log N)$ active qutrits for one memory access. Therefore, the BB-QRAM saves physical resources and energy compared to the fanout QRAM \cite{nielsen2001quantum}. The FF-QRAM is a circuit-based QRAM, which could be used in the state preparation step of a quantum algorithm. The FF-QRAM can encode the data into not only the basis state but also the amplitudes. After the circuit of a FF-QRAM, a quantum database will be generated and it can be the input of other quantum algorithms. 
%
%Although there are existing designs of QRAMs, but a scalable and workable implementation of a QRAM has not been achieved yet. In fact, the feasibility of an efficient QRAM is also contriversial \cite{ciliberto2018quantum}. This is one of the severest challenge to the real-world application of the quantum algorithms. However, we believe it is a problem that can be solved in the future. In this paper, we do not discuss the feasibility of a QRAM, and we assume that we have an efficient QRAM. It is the common sense in the discussion in the database area that a memory load and a memory store cost $O(1)$ time. Following \cite{kerenidis2017quantum, saeedi2019quantum}, in this paper, we assume a classical-write quantum-read QRAM. It takes $O(1)$ time to store a classical data point. Also, it takes $O(1)$ time to accept a superposition of addresses and return a superposition of the corresponding data points just like the above example. 
%
%\subsection{Application of a Quantum Range Query}\label{application}
%
%The first application is for the label binning in quantum machine learning. Label binning is a useful tool in machine learning. Assume there is a classification task with a training dataset $\{(x_1, y_1),\cdots,(x_N, y_N)\}$ where for each $i\in[1,N]$, $x_i$ is the feature vector and $y_N$ is a continues label. There are many studies show that to pack labels into bins can improve the accuracy of the label prediction. In \cite{dougherty1995supervised}, Dougherty et.al. introduced the equal-width binning, which is to bin the labels into $k$ equal-sized bins, where $k$ is a user parameter. They conducted experiments on 16 datasets to show that the label binning can improve the accuracy of Naive Bayes. In \cite{xue2017efficient}, Xue et.al. used equal-size binning to bin the labels into $k$ bins. They conducted experiments to show that the label binning can improve the accuracy of SVM and obtained the best performance when the bin size is set to $O(N^{1/3})$. They pointed out that $k$ will affect the quality of the result. In \cite{berg2021deep}, Berg et.al. used the neural network to do image classification. They did three tasks: Age estimation, head pose estimation and historial image dating. In the experiment, two of the three tasks were improved by label binning. They also claimed that $k$ has an impact on the prediction performance, and it is difficult to select $k$ for a given problem without extensive parameter search. 
%
%The above studies are based on the classical machine learning. We can learn that many machine learning algorithm can be improved by label binning in some scenarios, so it is reasonable to consider it may also improve the accuracy of quantum machine learning algorithms. For example, to train a quantum model, there is an existing methods called the single-shot training \cite{adhikary2020supervised}. To train a classical model, we input $(x_i, y_i)$ one by one and $N$ iterations are needed in an epoch. In single-shot training, we generate a superposition of all the $x_i$ with the same label $y_i$ and input the data in one iteration, so an epoch contains only $k$ iterations, where $k$ is the number of bins. We can first insert all the $(x_i, y_i)$ by $INSERT(y_i, x_i)$, where the continues label $y_i$ is the key and the feature vector $x_i$ is the record. To obtain such a superposition, we can make a range query of the bin boundaries to the quantum B+ tree. By existing methods like \cite{long2001efficient}, we encode each data points into quantum bits one by one, and it takes $O(N/k)$ time. By a range query to a quantum B+ tree, we only need $O(\log_B N)$ time.
%
%The second application is for a range filter of a recommendation system. For example, a recommendation system like \cite{gupta2013location, covington2016deep} usually has two steps. The first step is to select a small part of the all the items as the candidates. The second step is to use a model (e.g., a neural network) to predict the scores of the items for a user. For example, assume that we want the system recommend us a movie from 1990 to 1999. Now we have a model like \cite{biancalana2011context} to predict the score of the movie for a user. The first step is to select all the $k$ movies from 1990 to 1999 from the database with $N$ movies to obtain $\{movie_1, movie_2,\cdots,movie_k\}$, which costs $O(\log N + k)$ time . The second step is that for each $movie_i$, we use the model to predict the score $s(movie_i)$ for recommendation.  Assume the model prediction costs $T$ time for a movie, then it totally costs $O(kT)$ time. Therefore, the classical recommendation system costs $O(\log N + k + kT)$ time. Now consider a quantum system for the movie recommendation. Given that all the movies have been stored in the quantum B+ tree, we can obtain the $k$ movies in quantum bits by a quantum range query to the quantum B+ tree in $O(\log_B N)$ time: $$QUERY(1990, 1999)=\frac{1}{\sqrt{k}}\sum_{i=0}^{k-1}\ket{i}\ket{movie_i}.$$ Then, with a quantum model, we can predict the score of all the movies in $T$ time: $$\frac{1}{\sqrt{k}}\sum_{i=0}^{k-1}\ket{i}\ket{movie_i}\ket{0}\rightarrow \frac{1}{\sqrt{k}}\sum_{i=0}^{k-1}\ket{i}\ket{movie_i}\ket{s(movie_i)}.$$ Therefore, the quantum recommendation system only needs $O(\log_B N +T)$ time. A multi-dimensional example is location-based restaurant recommendation in \cite{gupta2013location}. If we use a classical range tree to index the locations and we have a model which predict the score of a restaurant in $T$ time, the classical recommendation system costs $O(\log^2 N + k + kT)$ time. With a quantum range tree, it can predict the scores in $O(\log^2_B N +T)$ time.
%
%Another example is the time-periodic-biased KNN in \cite{campos2010simple}. In this paper, Campos et.al. studied how to use KNN to do movie recommendations. They found that it can improve the accuracy to only consider the rating datasets from the last month before the recommendation time in different years.  That means they need to select the records produced in the same month but different years. Given a B+ tree containing all the movies sorted by the dates in the year, the calculation costs $O(\log_B N + N/12)$ time since the range query returns $N/12$ records on average. However, if we can use a quantum range query, we can select the records in $O(\log_B N)$ time. Note that there is an existing $O(d^3)$ quantum KNN algorithm \cite{ruan2017quantum} where $d$ is the dimension of the feature vector. Therefore, the whole process only costs $O(\log_B N + d^3)$. In the most cases, $d$ is much smaller than $N$. Assume $d=O(\log N)$, then we can say that the quantum time-periodic-biased KNN is exponentially faster than its classical competitor.











